Improved Decoding of Expander Codes

We study the classical expander codes, introduced by Sipser and Spielman \cite{SS96}. Given any constants $0< \alpha, \varepsilon < 1/2$, and an arbitrary bipartite graph with $N$ vertices on the left, $M < N$ vertices on the right, and left degree $D$ such that any left subset $S$ of size at most $\alpha N$ has at least $(1-\varepsilon)|S|D$ neighbors, we show that the corresponding linear code given by parity checks on the right has distance at least roughly $\frac{\alpha N}{2 \varepsilon }$. This is strictly better than the best known previous result of $2(1-\varepsilon ) \alpha N$ \cite{Sudan2000note, Viderman13b} whenever $\varepsilon < 1/2$, and improves the previous result significantly when $\varepsilon $ is small. Furthermore, we show that this distance is tight in general, thus providing a complete characterization of the distance of general expander codes. Next, we provide several efficient decoding algorithms, which vastly improve previous results in terms of the fraction of errors corrected, whenever $\varepsilon < \frac{1}{4}$. Finally, we also give a bound on the list-decoding radius of general expander codes, which beats the classical Johnson bound in certain situations (e.g., when the graph is almost regular and the code has a high rate). Our techniques exploit novel combinatorial properties of bipartite expander graphs. In particular, we establish a new size-expansion tradeoff, which may be of independent interests.

==> PreSec3and4.tex <==

\section{Improved Decoding for large expansion}
Let $\mathcal{C}$ be the expander code of a $(\alpha N, (1-\eps)D)$-expander. Consider the following algorithm modified from \cite{Viderman13b}:
\begin{enumerate}
\item Choose a parameter $k$ and thus $\mathcal{C}$ is a $(k \alpha N, (1-k \eps)D)$-expander.
\item Let $h_0=(1-2k \eps)D$ and $R_0=\{\text{all unsatisfied parties}\}$.
\item $L'(0)=\emptyset$.
\item $R'(0)=R_0$, $t=0$.

\item While $\exists i \in [N] \setminus L'(t)$ s.t. $|N(i) \cap R'(t)| \geq h_t$ do
\begin{enumerate}
    \item $L'(t+1)=L'(t) \cup \{i\}$.
    \item $R'(t+1)=R'(t) \cup N(i)$.
    \item $t=t+1$.
\end{enumerate}
\item $h_t$ is defined as follows: if $|L'(t)| \leq k \alpha N$ then $h_t=h_0$; otherwise $h_t=(1-2\frac{|L'(t)|}{\alpha N}\eps)D$.
\end{enumerate}

We want to bound $|L'(t)|$ for all $t$ by setting an appropriate $|Corr|$ which is the size of the corrupted bits. First we can show that if the above algorithm stops, then the order of adding $i \in [N]$ to $L'(t)$ does not matter, and we will always end up with the same set $L'(t)$ in the end. Thus, define $Corr_0 = \{i \in Corr | |N(i) \cap R_0| \geq h_0 \}$ and assume that $|Corr_0| \leq k \alpha N$ (we'll later show this assumption holds), WLOG we can assume we add $Corr_0$ to become $L'(0)$ in the first step and continue from there. Now if $|L'(t)| \leq k \alpha N$ for all $t$ then we are already done. Otherwise at some point the size grows larger than $k \alpha N$. We borrow the following claim (Claim 4.6) from \cite{Viderman13b}:

\begin{claim}
\[|N(Corr_0) \setminus R_0| \leq (D-h_0)|Corr_0| -|R_0|+h_0 |Corr|.\]
\end{claim}

Now before $|L'(t)|$ reaches $k \alpha N$, the size of $N(L'(t))$ grows by at most $D-h_0$ each time, after that it grows by at most $D-h_t$ each time. So we have the follow inequalities.

\begin{align*}
    (1-\frac{|L'(t)|}{\alpha N}\eps)D |L'(t)| & \leq |N(L'(t))| \leq |R_0|+|N(Corr_0) \setminus R_0|+\sum_{i=1}^{t}(D-h_{t-1}) \\
    & \leq (D-h_0)|Corr_0|+h_0 |Corr|+(D-h_0)(k \alpha N-|Corr_0|)+\frac{2\eps D}{\alpha N} \sum_{j=k\alpha N}^{|L'(t)|-1}j\\
    & \leq 2k^2 \eps D \alpha N +(1- 2 k \eps) D |Corr|+\frac{2\eps D}{\alpha N} \frac{|L'(t)|^2-(k\alpha N)^2}{2} \\
    & = 2k^2 \eps D \alpha N +(1- 2 k \eps) D |Corr|+\frac{\eps D}{\alpha N}(|L'(t)|^2-(k\alpha N)^2).
\end{align*}

Set $|L'(t)|=x$ and simplify, we get
\[x - \frac{2 \eps}{\alpha N} x^2 \leq k^2 \eps  \alpha N+(1- 2 k \eps)  |Corr|.\]

Note that the left hand side is maximized at $x=\frac{\alpha N}{4 \eps}$ with a value of $\frac{\alpha N}{8 \eps}$. Thus as long as we start with $|L'(0)| < \frac{\alpha N}{4 \eps}$ and set $|Corr|$ to be such that $k^2 \eps \alpha N+(1- 2 k \eps)  |Corr| < \frac{\alpha N}{8 \eps}$ we can bound $|L'(t)|$ by $\frac{\alpha N}{4 \eps}$.

Thus, roughly we can set $k^2 \eps \alpha N+(1- 2 k \eps)  |Corr| = \frac{\alpha N}{8 \eps}$ and $|Corr|=\frac{\frac{\alpha N}{8 \eps}-k^2 \eps \alpha N}{1- 2 k \eps}$. This is maximized when setting $k=\frac{1-\frac{1}{\sqrt{2}}}{2\eps}$, where we get $|Corr|=(2-\sqrt{2})\frac{\alpha N}{4 \eps}$. Notice for this setting we have $|Corr|=k \alpha N$ and thus $|Corr_0| \leq |Corr| = k \alpha N$. Furthermore $k \alpha N < \frac{\alpha N}{4 \eps}$.

The proof that $Corr \subseteq |L'(t)|$ can use the same argument as the Proof of Proposition 4.3 in \cite{Viderman13b}, and by noticing that $h_0 \geq h_t$.

\section{The case of $\eps < \frac{1}{2\sqrt{2}}$} \textcolor{red}{There is a problem here.}
In the above analysis, set $k=1$ and the final inequality becomes 

\[x - \frac{2 \eps}{\alpha N} x^2 \leq  \eps  \alpha N+(1- 2 \eps)  |Corr|.\]

When $\eps \leq \frac{1}{2\sqrt{2}}-c$ for any constant $c>0$, we can set $|Corr|$ to be a small enough $\Theta(\alpha N)$ (in particular, $|Corr| < \frac{\alpha N}{2}$) s.t. $ \eps \alpha N+(1- 2  \eps)  |Corr| < \frac{\alpha N}{8 \eps}$.

We now check the following conditions:

\begin{enumerate}
\item $|Corr_0| \leq |Corr| <  \alpha N$ holds, so that we can use Claim 4.6 from \cite{Viderman13b}.
\item $|L'(0)|=|Corr_0| \leq |Corr| \leq \frac{\alpha N}{2} < \frac{\alpha N}{4 \eps}$ holds, so that we start with a $|L'(0)|$ smaller than the value $\frac{\alpha N}{4 \eps}$ which maximizes $x - \frac{2 \eps}{\alpha N} x^2$.
\item $ \eps \alpha N+(1- 2  \eps)  |Corr| < \frac{\alpha N}{8 \eps}$ holds by our choice of $|Corr|$.
\end{enumerate}

Thus we still have the bound $|L'(t)| \leq max\{\alpha N, \frac{\alpha N}{4 \eps}\}$.


==> backup.tex <==
\iffalse
\section{}
We give a finding erasure algorithm and then use the Decoding from erasures algorithm in Theorem \ref{thm:vidermandecfromerasures}.

\subsection{Find Erasures}
Consider the following algorithm:

Fix some parameter $x$ which we will choose later, such that $|Corr| =x \alpha N$. 
In this section we want to maximize $|Corr|$ so we assume $x \geq 1$. Define $h_c=(1-2\frac{|Corr|}{\alpha N}\eps)D=(1-2x \eps)D$. 


\begin{enumerate}
\item Let $R_0=\{\text{all unsatisfied parities}\}$.
\item $L'(0)=\emptyset$.
\item $R'(0)=R_0$, $t=0$.

\item While $\exists i \in [N] \setminus L'(t)$ s.t. $|N(i) \cap R'(t)| \geq h_c$ do
\begin{enumerate}
    \item $L'(t+1)=L'(t) \cup \{i\}$.
    \item $R'(t+1)=R'(t) \cup N(i)$.
    \item $t=t+1$.
\end{enumerate}
\end{enumerate}


We have the following claims:

\begin{claim}
\label{claim:CorrIsInL'1}
When the above algorithm stops, we have $Corr \subseteq L'(t)$.
\end{claim}
We use a similar proof to the proof of 4.3 in \cite{Viderman13b}. 
\begin{proof}
Suppose there is a subset $B \subseteq Corr$ such that $B$ is not contained in $L'(t)$. 
By the expansion property, the set of unique neighbors of $B$ has size at least $(1-2x\eps)D|B| = h_c|B|$. 
By the algorithm, every vertex in $B$ has less than $h_c$ neighbors in $R'(t)$. 
So $B$ has some unique neighbor $v$ not in $R'(t)$.
Since $R'(t)$ contains all the neighbors of $Corr \backslash B$, $v$ has to be unsatisfied. 
Then it has to be included in $R'(0)$ and thus in $R'(t)$. 
This is a contradiction.
\end{proof}

Define $Corr_0 = \{i \in Corr \mid |N(i) \cap R_0| \geq h_c \}$, Without loss of generality we can assume we add $Corr_0$ to become $L'(0)$ in the first step and continue from there. 
This assumption is true by the following claim.
%\begin{claim}
%For every iteration $t$, if there are more than $1$ vertices in the left such that all of them have at least $h_c$ neighbors in $R'(t)$, then all %these vertices will be added into $L'$ after all the iterations.
%\end{claim}
%\begin{proof}
%Let $u$ be such a vertex which is not added to $L'$ in iteration $t$.
%So $|N(u) \cap R'(t)| \geq h_c$.
%Notice that $R'(t) \subseteq R'(t+1)$ for every $t$. 
%Hence for every iteration $t'$ after $t$, we have $|N(u) \cap R'(t')| \geq h_c$.
%As we always add one vertex to $L'$ in each iteration, $u$ will be added to $L'$ before the end of the iterations.
%\end{proof}
%We can deduce the following claim.
\begin{claim}
\label{claim:L'allsame}
In every iteration, if there are multiple vertices that can be added to $L'$ and we choose one of them arbitrarily, then we always get the same $L'$ after all the iterations.
\end{claim}
\begin{proof}
Consider two different procedures such that they choose different vertices to add to $L'$ in their iterations.
Suppose the they get two different $L'$, saying $L_1$ for the first procedure and $ L_2$ for the second.
Without loss of generality assume $L_1 \backslash L_2 \neq \emptyset$.
Let $u$ be the vertex which is in  $L_1 \backslash L_2$ and is the one added first among them in procedure 1.
Then all the vertices in $L_1$ added before $u$ is in $L_2$. 
So for procedure 2 we should have $|N(u)\cap R'| \geq h_c$.
Thus $u$ has to be added to $L_2$ in procedure 2.
This is a contradiction.
Therefore $L_1 = L_2$.
\end{proof}
%\xnote{I don't think the above paragraph follows from the previous claim in a straightforward manner. Specifically, if we add vertices in different orders then the set of vertices that can be added in each iteration will also change. We need to explain this in more details. In my view, we should make this an independent claim.}


Next we borrow the following claim   from \cite{Viderman13b}:
\begin{claim}[Claim 4.6 from \cite{Viderman13b}]
\[|N(Corr_0) \setminus R_0| \leq (D-h_c)|Corr_0| -|R_0|+h_c |Corr|.\]
\end{claim}

Now we want to bound $|L'(t)|$. 

\begin{claim}
\label{claim:boundOnL'(t)}
For every $x$ such that $x < \frac{1}{6\eps}$ and $x\leq \frac{1-2\eps}{2\eps}$, we have $|L'(t)| < \frac{1-2 \eps x}{2 \eps} \alpha N$.
\end{claim}

\begin{proof}
Let $k_0 = \frac{1}{3\eps}$.
Suppose this is not true, for some $t$, If for all $t$ we have $|L'(t)| < k_0  \alpha N$ then we are already done. 
Now before $|L'(t)|$ exceeds $k_0  \alpha N$.
Let $|L'(t)|=k \alpha N$.
When $k\geq 1$, we have 
\begin{align*}
    (1-\frac{|L'(t)|}{\alpha N}\eps)D |L'(t)| & \leq |N(L'(t))| \leq |R_0|+|N(Corr_0) \setminus R_0|+(D-h_c)(|L'(t)|-|Corr_0|) \\
    & \leq (D-h_c)|Corr_0|+h_c |Corr|+(D-h_c)(|L'(t)|-|Corr_0|)\\
    & =(D-h_c)|L'(t)| +h_c |Corr| =2x \eps D|L'(t)|+(1-2x \eps)D|Corr|\\
\end{align*}
Plug into the above inequality and simplify, we get 
\[(1-k \eps)k \leq 2 x \eps k+(1-2 x \eps) x.\]
and
\[(1-2\eps x)k -\eps k^2 \leq x-2 \eps x^2.\]


The LHS is maximized at $k_0= \frac{1-2 \eps x}{2 \eps}$ with a value of $\frac{(1-2 \eps x)^2}{4 \eps}$.
Since $x\leq  \frac{1-2\eps}{2\eps}$, we have $k_0 \geq 1$.
On the other hand, as $x < \frac{1}{6\eps}$,   it must be $\frac{(1-2 \eps x)^2}{4 \eps} > x-2 \eps x^2$. 
So $k$ has to be less than $k_0$.  



%The LHS is maximized at $k_0= \frac{1-2 \eps x}{2 \eps}$ with a value of $\frac{(1-2 \eps x)^2}{4 \eps}$. 
%Hence as long as we have $|Corr_0| \leq |Corr| \leq k_0 \alpha N$ and $\frac{(1-2 \eps x)^2}{4 \eps} > x-2 \eps x^2$ we can bound $|L'(t)|$ by $k_0 \alpha N$. Solving this gives that $x < \frac{1}{6\eps}$.

\end{proof}




\begin{theorem}

Let $G$ be a $(\alpha N, (1-\eps) D)$ expander with $\eps \leq 1/6 $.  The expander code defined by $G$ has an efficient decoding algorithm with decoding radius $(\frac{1}{6\eps}-o(1))\alpha N$.

\end{theorem}

\begin{proof}
Consider that we are decoding from erasures in Corr, where $|Corr| = x\alpha N$.
We first run the finding erasures algorithm.
By Claim \ref{claim:CorrIsInL'1}, we know Corr is contained in $L'(t)$.
When $\eps \leq \frac{1}{6}$, if $ x\alpha N$ is any number less than $\frac{\alpha N}{6 \eps} $, then by Claim \ref{claim:boundOnL'(t)}, we must have $|L'(t)| \leq \frac{1}{3\eps} \alpha N$.

By Lemma \ref{lem:expansion_larger}, the expander is a $(\frac{1}{3\eps} \alpha N, \frac{2}{3}D)$ expander. So it is also a $(\frac{1}{3\eps} \alpha N, \frac{1}{3}D)$ unique expander.
Hence by Theorem \ref{thm:vidermandecfromerasures}, using $L'(t)$ and the corrupted codeword, we can decode correctly.


\end{proof}

\fi


\section{Parallel algorithm}
Let $\mathcal{C}$ be the expander code of a $(\alpha N, (1-\eps)D)$-expander. We know the distance is $\frac{\alpha N}{2\eps}$. Consider the following algorithm:
\begin{enumerate}
\item In parallel, flip each variable whose $(1-2\eps)D$ neighbors are not satisfied. 
\item Repeat until no such variable ramains.
\end{enumerate}

Our main result is the decoding distance.
\begin{claim}
For any $\eps<1/4$, the above algorithm corrects more than $(\frac{1-2\eps}{4\eps}-o(1)) \cdot \alpha$ fraction errors. \end{claim}
Remark: $\frac{1-2\eps}{4\eps}$ is always larger than $\frac{1-3 \eps}{1-2\eps}$ for $\eps<1/4$.

\begin{proof}
We follow the anaylsis of Theorem 11 \cite{SS96} to argue that the errors reduce in every round. Let  $V$ denote the set the corrupted variables on the L.H.S. We use $F \subset V$ to denote those corrupted variables donot flip in this round and $C \subset \ov{V}$ to denote the uncorrupted variables get flipped in this round. So we wanna show $|V| > |F| + |C|$.

First of all, we wanna claim $|V \cup C| < k \cdot  \alpha n$ for \[k=\frac{1-2\eps}{2\eps} - o(1).
\]
Without loss of generality, we assume $|V \cup C|=k \alpha n$ and $\delta$ is the expansion of $V$: $N(V)=\delta D \cdot |V|$. Because each variable in $C$ contributes at most $2 \epsilon D$ new neighbors to this union, 
\[
|N(V \cup C)| \le \delta D \cdot |V| + 2\epsilon D \cdot (k \alpha n - |V|).
\]
At the same time, by the guarantee of expander graphs,
\[
|N(V \cup C)| \ge (1 - k \epsilon) D \cdot k \alpha n.
\]
So we combine them together and cancel $D$ to obtain
\[
(k - k^2 \epsilon - 2 k \epsilon) \alpha n \le (\delta - 2 \epsilon) |V|.
\]
Since $\delta \le 1$, $|V| \ge \frac{k - k^2 \epsilon - 2 k \epsilon}{1-2\eps} \alpha n$, which is contradicted to the assumption of $|V|$ given \[k - k^2 \epsilon - 2 k \epsilon=(1-2 \epsilon)^2/4\eps - o(1)
\] for our choice of $k$. So $|V \cup C| < k \alpha n$ gives us the lower bound on $|N(V \cup C)|$:
\begin{equation}\label{eq:neighbors_V_C}
(1 - k\eps)D \cdot (|V|+|C|) \le |N(V \cup C)| \le \delta D \cdot |V| + 2 \epsilon D \cdot |C|.
\end{equation}

Now we bound $\delta D \cdot |V|$ using $F$. Note that each variable in $F$ does not get flipped because it shares at least $2 \eps D$ neighbors with other variables in $V$. In the worst case, these $2 \eps D$ neighbors are shared with other variables in $F$. So $F$ contribute at most $(1-\eps)D \cdot |F|$ neighbors. Then we have
\[
\delta D \cdot |V| \le (1 - \eps) D \cdot |F| + D(|V|-|F|)=D(|V|-\eps|F|).
\]
If we plug this into \eqref{eq:neighbors_V_C}, we conclude
\[
(1 - k \eps)D \cdot (|V|+|C|) \le D(|V| - \eps|F|)+ 2\eps D \cdot |C|.
\]
This shows 
\[
(1 - k \eps - 2 \eps) |C| + \eps |F| \le k \eps \cdot |V|.
\]
Given $k \in (1,\frac{1-2\eps}{2\eps})$, we have $k \eps < (1-k \eps - 2 \eps)$. This gives $|V|>|C|+|F|$. \textcolor{red}{This line is problematic.}
\end{proof}

It may be worth to check previous work \cite{FMSSW07,Viderman13,Viderman13b} and the reference therein about the improvement upon \cite{SS96}.


\section{Adaptive Threshold}
We consider using multiple thresholds in this section. Let $x \alpha N$ denote the size of corruption $F$. For ease of exposition, we fix $x=1/5\eps$ in the rest calculation.

Let $1-\gamma x$ be the expansion of $F$ such that $\Gamma(F)=(1-\gamma x)D \cdot x \alpha N$. We choose the first threshold to be $(1-C \gamma x)D$ for some $C \in [2,\frac{3+\sqrt{5}}{2}-o(1)]$ (we will see the calculation of $C$ later).

\begin{remark}
By the definition, $\gamma \in [0,\eps]$ and $C \in [2,2.6]$. While we donot know $\gamma$ at the beginning, we could always enumerate $\gamma$ in a polynomial time algorithm (at least for the first threshold).
\end{remark}

Let $R_0$ be the wrong parity checks on the left hand side and $L_0=\{v | \Gamma(v) \cap R_0 \ge (1-C \gamma x)D\}$. We still use $C_0 = L_0 \cap F$ to denote corrupted vertices in $L_0$. For convenience, let $\delta \alpha N$ denote the number of wrong marked vertices in $L_0$, i.e., $|L_0 \setminus F|$.

\begin{claim}
Given our parameter $x\eps=1/5$, $\gamma$, and $C=\frac{3+\sqrt{5}}{2} - o(1)$, $\delta \le \frac{\frac{3}{5}-\frac{3+\sqrt{5}}{2} \cdot \gamma x}{2\eps} - o(1)$.
\end{claim}
\begin{proof}
We will consider the expansion of $L_0 \cup F$, whose size is $(\delta + x) \alpha N$. By Lemma~\ref{lem:expansion_larger},
it is at least $\bigg( 1 - (\delta + x)\eps \bigg) D \cdot (\delta+x) \alpha N$. On the other hand, we know $\Gamma(F)=(1-\gamma x)D \cdot x \alpha N$ by the definition of $\gamma$ and each vertex in $L_0 \setminus F$ will contribute at most $C \gamma x D$ vertices to $\Gamma(L_0 \cup F)$. To show the existence of $\delta$, we provide a $\delta$ such that (after normalizing $D \alpha N$)
\[
(1 - (\delta+x)\eps) \cdot (\delta + x) \ge (1-x \gamma)x + C\gamma x \delta.
\]
This is equivalent to show
\[
0 \ge \eps (\delta + x)^2 - \delta - \gamma x^2 + C \gamma x \delta = \eps \delta^2  + (2\eps x +C \gamma x - 1)\delta + (\eps-\gamma)x^2.
\]
So we only need to show the right quadratic polynomial has two roots. Namely,
\begin{equation}\label{eq:bsquare4ac}
(2\eps x +C \gamma x - 1)^2 - 4 \eps \cdot (\eps-\gamma)x^2 > 0
\end{equation}
such that the above quadratic equation of $\delta$ has two roots.

We set $\beta:= \gamma x$ and plug $\eps x=1/5$ to simplify \eqref{eq:bsquare4ac} as
\[
(C \beta - 3/5)^2 - 4/25 + 4\beta/5 = C^2 \beta^2 + (4/5 - 6C/5) \beta + 1/5 > 0.
\]
Since $\gamma$ could be any number in $[0,\eps]$, we choose $C$ such that the above inequality is always true. Namely we want it does not have a root:
\[
0 > (4/5-6C/5)^2 - 4 C^2 /5 = 36 C^2 /25 - 48 C/25 + 16/25 - 4C^2/5.
\]
So we get
\[
C^2 - 3C + 1 < 0 \Rightarrow C \in \left( \frac{3-\sqrt{5}}{2},\frac{3+\sqrt{5}}{2} \right).
\]

Thus we choose $C=\frac{3+\sqrt{5}}{2} - o(1)$ and get $\delta = \frac{2\eps x + C \gamma x - 1}{2\eps} \pm o(1)$.
\end{proof}
\begin{corollary}
Given $x \ge 1$ such that $x \eps=1/5$, let $F$ be the set of flipped coordinates of size $x \alpha N$. If $N(F)=(1-\beta)D \alpha N$ for $\beta:=\gamma x$ in $[0,1/20] \cup [0.18,0.2]$, we can choose $C$ properly such that $|L_0 \setminus C_0| < |C_0|$. 

This means we only need to flip all bits in $L_0$ to reduce the error for particular values of $\beta$.
\end{corollary}

\begin{proof}
From the above calculation, we know $|L_0 \setminus C_0| \le \delta \alpha N$ for 
\[
\delta \le \frac{1-2\eps x - C \gamma x - \sqrt{(1-2\eps x - C \gamma x)^2 - 4 \eps^2 x^2 + 4 \eps x \gamma x}}{2\eps}.
\]
After plugging $\eps x=1/5$ and $\beta:=\gamma x$, this becomes
\[
\delta \le \frac{\frac{3}{5} - C \beta - \sqrt{(\frac{3}{5} - C \beta)^2 - \frac{4}{25} + \frac{4}{5} \beta}}{2\eps}. 
\]
At the same time, $C_0/\alpha N$ is at least
\[
x \cdot (1 - 2 \beta / C \beta) = \frac{1-2/C}{5 \eps}.
\]
So we wanna show for some $\beta$,
\[
\frac{\frac{3}{5} - C \beta - \sqrt{(\frac{3}{5} - C \beta)^2 - \frac{4}{25} + \frac{4}{5} \beta}}{2\eps} \le \frac{1-2/C}{5 \eps}.
\]
When $\beta \le 1/20$, we could choose $C=1/5\beta$, that is at least 4. So it becomes to verify
\[
\frac{\frac{3}{5} - \frac{1}{5} - \sqrt{ \frac{4}{5} \beta}}{2\eps} \le \frac{1-10 \beta}{5 \eps}.
\]
We verify it as
\[
1 - \sqrt{5 \beta} \le 1 - 10 \beta.
\]
For $\beta \in [0.18,0.2]$, we could choose $C \in  [2.4,2.6]$ to show the same thing.
\end{proof}

\subsection{Attempt 0}
\textcolor{red}{Xue: I donot know what is the best way to finish the argument. Here is some naive attempt.}
Let us consider $C \ge 2.2$ and $x=1.1$ such that we only need to reset the threshold once. 

%By the Markov's inequality, \[|F \setminus C_0|/|F| \le \frac{2}{C} = \frac{4}{3 +\sqrt{5}} = 3-\sqrt{5} \text{ and } |C_0|/|F| \ge \sqrt{5} - 2.\] This indicates $|F \setminus C_0|<\alpha N$. 

A natural choice of the threshold is $h_1=(1-2\eps)D$ (\textcolor{red}{Xue: One question here --- shall we choose $h_1$ that depends on $\gamma$?})  and apply the algorithm in Section~\ref{sec:improved}. To finish the argument, we wanna show the existence of $\delta_1$ such that
\[
(1 - (x+\delta + \delta_1)\eps) \cdot (x+\delta + \delta_1) \ge (1-\gamma x) x + C \gamma x \delta + 2 \eps \delta_1
\]
By the same simplification, we get
\[
\delta + \delta_1 - (x+\delta + \delta_1)^2 \eps \ge - \gamma x^2 + C \gamma x \delta + 2\eps \delta_1.
\]
For $x=1$ and $\eps=1/5$, we get
\[
0 > (1+\delta+\delta_1)^2 /5 - \delta - \delta_1 - \gamma + C \gamma \delta + \frac{2}{5} \delta_1 = \delta_1^2/5 + (2/5 + 2 \delta/5  -1 + 2/5)\delta_1 + (1+\delta)^2/5 - \gamma + C \gamma \delta.
\]
So our goal is to show $\delta_1$, which depends on $\delta,C,\gamma$, such that
\[
0 > \delta_1^2/5 + (2 \delta/5  -1/5)\delta_1 + (1+\delta)^2/5 - \gamma + C \gamma \delta.
\]

\subsection{OLD material}
We consider use two thresholds $h_0$ and $h_1$. Let $x \alpha N$ be the upper bound of $Corr$ and $k \alpha N$ be the upper bound of $L(t)$. We plan to set $h_0 < (1-2x \eps)D$ (say $h_0=(1-3x \eps)D$) such that $bad$ is small and $h_1 > (1-2x \eps)D$. So the inequality becomes
\[
(1-k \eps)k \le R_0 + N(Corr_0)\setminus R_0 + N(L_0) \setminus ( N(Corr_0) \cup R_0) + (D-h_1) \cdot (k-L(0))
\]
One way to upper bound the right hand side is
\[
h_0 \cdot |Corr| + (D-h_0) \cdot |Corr_0| + (D-h_0) \cdot |L(0) \setminus Corr_0| + (k - L(0)) \cdot (D- h_1) = h_0 \cdot |Corr| + (h1-h_0) \cdot |L(0)| + (D-h_1)k.
\]

As a first step, we wanna bound $L(0)$. Let $\delta$ denote the fraction of $L(0)\setminus |Corr_0|$. In the worst case --- $Corr_0=Corr$, we could consider
\[
(1 - (x+\delta)\eps) \cdot (x+\delta) \le x + (1-h_0) \cdot \delta.
\]
However, to upper bound $\delta$, this seems to force $x \eps \le 1/6$ for $h_0 \le (1-2x \eps)$.

\section{Parallel algorithm}
Let $\mathcal{C}$ be the expander code of a $(\alpha N, (1-\eps)D)$-expander. We know the distance is $\frac{\alpha N}{2\eps}$. Consider the following algorithm:
\begin{enumerate}
\item In parallel, flip each variable whose $(1-2\eps)D$ neighbors are not satisfied. 
\item Repeat until no such variable ramains.
\end{enumerate}

Our main result is the decoding distance.
\begin{claim}
For any $\eps<1/4$, the above algorithm corrects more than $(\frac{1-2\eps}{4\eps}-o(1)) \cdot \alpha$ fraction errors. \end{claim}
Remark: $\frac{1-2\eps}{4\eps}$ is always larger than $\frac{1-3 \eps}{1-2\eps}$ for $\eps<1/4$.

\begin{proof}
We follow the anaylsis of Theorem 11 \cite{SS96} to argue that the errors reduce in every round. Let  $V$ denote the set the corrupted variables on the L.H.S. We use $F \subset V$ to denote those corrupted variables donot flip in this round and $C \subset \ov{V}$ to denote the uncorrupted variables get flipped in this round. So we wanna show $|V| > |F| + |C|$.

First of all, we wanna claim $|V \cup C| < k \cdot  \alpha n$ for \[k=\frac{1-2\eps}{2\eps} - o(1).
\]
Without loss of generality, we assume $|V \cup C|=k \alpha n$ and $\delta$ is the expansion of $V$: $N(V)=\delta D \cdot |V|$. Because each variable in $C$ contributes at most $2 \epsilon D$ new neighbors to this union, 
\[
|N(V \cup C)| \le \delta D \cdot |V| + 2\epsilon D \cdot (k \alpha n - |V|).
\]
At the same time, by the guarantee of expander graphs,
\[
|N(V \cup C)| \ge (1 - k \epsilon) D \cdot k \alpha n.
\]
So we combine them together and cancel $D$ to obtain
\[
(k - k^2 \epsilon - 2 k \epsilon) \alpha n \le (\delta - 2 \epsilon) |V|.
\]
Since $\delta \le 1$, $|V| \ge \frac{k - k^2 \epsilon - 2 k \epsilon}{1-2\eps} \alpha n$, which is contradicted to the assumption of $|V|$ given \[k - k^2 \epsilon - 2 k \epsilon=(1-2 \epsilon)^2/4\eps - o(1)
\] for our choice of $k$. So $|V \cup C| < k \alpha n$ gives us the lower bound on $|N(V \cup C)|$:
\begin{equation}\label{eq:neighbors_V_C}
(1 - k\eps)D \cdot (|V|+|C|) \le |N(V \cup C)| \le \delta D \cdot |V| + 2 \epsilon D \cdot |C|.
\end{equation}

Now we bound $\delta D \cdot |V|$ using $F$. Note that each variable in $F$ does not get flipped because it shares at least $2 \eps D$ neighbors with other variables in $V$. In the worst case, these $2 \eps D$ neighbors are shared with other variables in $F$. So $F$ contribute at most $(1-\eps)D \cdot |F|$ neighbors. Then we have
\[
\delta D \cdot |V| \le (1 - \eps) D \cdot |F| + D(|V|-|F|)=D(|V|-\eps|F|).
\]
If we plug this into \eqref{eq:neighbors_V_C}, we conclude
\[
(1 - k \eps)D \cdot (|V|+|C|) \le D(|V| - \eps|F|)+ 2\eps D \cdot |C|.
\]
This shows 
\[
(1 - k \eps - 2 \eps) |C| + \eps |F| \le k \eps \cdot |V|.
\]
Given $k \in (1,\frac{1-2\eps}{2\eps})$, we have $k \eps < (1-k \eps - 2 \eps)$. This gives $|V|>|C|+|F|$. \textcolor{red}{This line is problematic.}
\end{proof}

It may be worth to check previous work \cite{FMSSW07,Viderman13,Viderman13b} and the reference therein about the improvement upon \cite{SS96}.

\iffalse
We split $S$ into $k$ subsets $S_1,\ldots, S_k$ where each $S_i$ is of size at most $\gamma/2 \cdot N$. From the property of $G$, we know
\begin{equation}\label{eq:bound_S_i}
    |\Gamma(S_i)| \in [(1-\eps) d \cdot |S_i|, d \cdot |S_i|]
\end{equation}
and 
\begin{equation}\label{eq:bound_S_i_j}
        |\Gamma(S_i \cup S_j)| \in [(1-\eps) d \cdot |S_i \cup S_j|, d \cdot |S_i \cup S_j|].
\end{equation}
Now we lower bound $\Gamma(S_1\cup S_2 \cdots \cup S_k)$ by
\begin{align*}
    \sum_{i=1}^k |\Gamma(S_i)| - \sum_{i<j} |\Gamma(S_i) \cap \Gamma(S_j)| & = \sum_{i<j} |\Gamma(S_i \cup S_j)| - (k-2) \sum_i |\Gamma(S_i)| \\
    & \ge \sum_{i<j} (1-\eps) d \cdot |S_i \cup S_j| - (k-2) \sum_i d |S_i| \tag{by bounds in \eqref{eq:bound_S_i} and \eqref{eq:bound_S_i_j}}\\
    & = (1-\eps)d \cdot (k-1) \cdot |S| - (k-2)d |S|\\
    & = \left(1 - (k-1)\eps \right) d |S|.
\end{align*}
\end{proof}
\begin{remark}
One intriguing question is whether we could improve it using more levels in the approxiation of inclusion-exclusion formula. For example, when $|S|=3/2 \cdot \gamma N$, we could split it into 6 subsets of size $\gamma /4 \cdot N$ instead of 3 subsets of size $\gamma /2 \cdot N$. Then we have
\begin{align*}
    |\Gamma(S)| & \ge \sum_{i} |\Gamma(S_i)| - \sum_{i_1<i_2} |\Gamma(S_{i_1} \cap S_{i_2})| + \sum_{i_1<i_2<i_3} |\Gamma(S_{i_1} \cap S_{i_2} \cap S_{i_3})| - \sum_{i_1<i_2<i_3<i_4} |\Gamma(S_{i_1} \cap S_{i_2} \cap S_{i_3} \cap S_{i_4}|\\
    & = \sum_{i_1<i_2<i_3<i_4} |\Gamma(S_{i_1} \cup S_{i_2} \cup S_{i_3} \cup S_{i_4}| - 2 \sum |\Gamma(S_{i_1} \cup S_{i_2} \cup S_{i_3})| + 3 \sum |\Gamma(S_{i_1} \cup S_{i_2})| - 4\sum |\Gamma(S_i)|.
\end{align*}
But I didnot see a way to improve the parameter.
\end{remark}

\paragraph{Distance.} As suggested by Xin, \[
dist(C) \ge 
\min_{|\Gamma(T)| \le d/2 \cdot |T|} |T|.
\] 
Now we recalculate the distance.
\begin{enumerate}
    \item If $\frac{1/2}{\eps}$ is not an integer, we set $k=[\frac{1/2}{\eps}]+1$. By Lemma~\ref{lem:expansion_larger}, any subset of size $k \cdot \gamma/2 \cdot N$ has $|\Gamma(S)| \ge (1-(k-1)\eps) d |S|$. So the number of unique neighbors is $(1-2(k-1)\eps) d |S|>0$. Then we could add at least another $(1-2(k-1)\eps) |S|$ vertices to $S$ to kill all unique neighbors. So the distance is
    \[
    |S|+(1-2(k-1)\eps) |S| =
    \left( 1 + 1-2(k-1)\eps \right)\cdot k \cdot \gamma/2 \cdot N.
    \]
    \item If $\frac{1/2}{\eps}$ is an integer, by a similar calculation, the distance turns out to be exact
    \[
    (k+1) \cdot \gamma/2 \cdot N \text{ for } k=\frac{1/2}{\eps}.
    \]
\end{enumerate}

\section{Adaptive Threshold}
\textcolor{red}{This result is problematic unless we can upper bound $|corr\setminus corr_0|$.} Consider the following algorithm with an adaptive threshold $h_t$: $h_t=(1-2\eps)D$ for $L'(t) \le 2 \alpha N$ and $h_t = (1-\eps \cdot \frac{L'(t)}{\alpha N})D$ for $L'(t) > 2 \alpha N$.
\begin{enumerate}
\item Let $R_0=\{\text{all unsatisfied parities}\}$.
\item $L'(0)=\emptyset$.
\item $R'(0)=R_0$, $t=0$.

\item While $\exists i \in [N] \setminus L'(t)$ s.t. $|N(i) \cap R'(t)| \geq h_t$ do
\begin{enumerate}
    \item $L'(t+1)=L'(t) \cup \{i\}$.
    \item $R'(t+1)=R'(t) \cup N(i)$.
    \item $t=t+1$.
\end{enumerate}
\end{enumerate}

If Claims 5.1 and 5.2 hold, we  bound $L'(t)$ and $|Corr|$ given $\eps$. Let $k \alpha N$ be the upper bound of $L'(t)$. Similar to the above argument, let $h_0=(1-2\eps)D$ in the following calculation.
\begin{align*}
    (1- \frac{L'(t)}{\alpha N} \eps) \cdot D \cdot |L'(t)| \le & |N(L'(t))| \\
    & \le |R_0| + |N(Corr_0)\setminus R_0| + \sum_{j=2 \alpha N + 1}^{k \alpha N} (1-\eps \cdot \frac{L'}{\alpha N})D\\
    & \le (D-h_0) \cdot |Corr_0| + h_0 |Corr| + (D-h_0) \cdot (2 \alpha N - |Corr_0|) + \frac{\eps D}{\alpha N} \sum_{j=2\alpha N + 1}^{k \alpha N} j \\
    & \le (1-2\eps)D \cdot |Corr| + 2 \eps D \cdot 2 \alpha N + \frac{\eps D}{\alpha N} \cdot \frac{(k-2) \alpha N \cdot \big( (k+2) \alpha N + 1)}{2}
\end{align*}
We remove the common factor $D$ and normalize both sides by $\alpha N$ to get
\[
(1-k \eps) \cdot k \le (1-2 \eps) \frac{|Corr|}{\alpha N} + 4 \eps  +  \eps \frac{k^2 -4}{2} + \eps \frac{k-2}{\alpha N}.
\]
Then we omit the last term $\eps \frac{k-2}{\alpha N}$ to get
\[
\frac{|Corr|}{\alpha N} \ge \frac{k - 1.5 \eps k^2 - 2\eps }{1 - 2 \eps}.
\]
For $k=\frac{1}{3\eps}$, the right hand side is about $$\frac{\frac{1}{6\eps} - 2\eps}{1 - 2\eps}.$$
This is slightly better than $1/6\eps$ when $\eps < 1/6$.

One restriction of this calculation is that $k>2$ implies $\eps<1/6$.
\fi




==> backup1.tex <==
\section{Improved Unique Decoding}

Let $\mathcal{C}$ be an expander code defined by an $(\alpha N, (1-\eps)D)$ expander $\Gamma: [N] \rightarrow [M]$.

\subsection{Decoding algorithm for the case $\eps \in (1/6,1/4]$}
Consider Algorithm \ref{alg:FindingErasure} with a fixed threshold $\Delta = \eps$. 
Let the set of errors be $F$ and assume $|F| = x\alpha N$.

\begin{claim}
\label{claim:errors_in_L}
If $x \leq 1$, then when the algorithm stops, we have $F \subseteq L$.
\end{claim}

\begin{proof}
As $x\leq 1$, for every $B\subseteq F$, $|\Gamma(B)| \geq (1-\eps)D|B|$.
Hence $|\Gamma^1(B)| \geq (1-2\eps)D|B|$.
By Lemma \ref{lemma:all_errors_in_L}, we have $F\subseteq L$, when the algorithm stops.
\end{proof}


\begin{claim}
\label{claim:bound_L}
If $\eps \leq 1/4$, then for every $x < \frac{1-2\eps}{4 \eps} - O(1/N)$, $|L| \leq \frac{1-2 \eps}{2 \eps}\alpha N$, when the algorithm stops.

\end{claim}

Let $R_0$ be the set of unsatisfied checks.
Let $F_0$ be the set of errors such that for every $i\in F_0$, $|\Gamma(i)\cap R_0 |\geq (1-2\eps)D$.

\begin{proof}
Let  $L = k \alpha N \geq \alpha N$. 
By a similar argument to \cite{Viderman13b} we can have \textcolor{red}{Xue: Shall we call Lemma~\ref{lemma:L'allsame}?}
\begin{align*}
    (1-\frac{|L|}{\alpha N}\eps)D |L| - O(1)   \leq |\Gamma(L)| & \leq |R_0|+|\Gamma(F_0) \setminus R_0|+(D-h_c)(|L|-|F_0|) \\
    & \leq (D-h_c)|F_0|+h_c |F|+(D-h_c)(|L|-|F_0|)\\
    & =(D-h_c)|L| +h_c |F| \\
    &=2x \eps D|L|+(1-2x \eps)D|F|.
\end{align*}
Here the first inequality is due to Lemma \ref{lem:expansion_larger}. 
The second inequality is due to the following.
At the beginning we set $R = R_0$. 
Then by Lemma \ref{lemma:L'allsame}, we can consider that $L$ is generated by first adding all vertices in $F_0$ to $L$ and then add other vertices in $L$.
Right after adding $F_0$ to $L$, $R$ is at most $|R_0| + |\Gamma(F_0) \setminus R_0| $.
By adding each vertex in $L\setminus F_0$, the size of $R$ increases by at most $D-h_c$.
The third inequality is since $  |R_0|+|\Gamma(F_0) \leq (D-h_c)|F_0|+h_c |F|$ by Claim 4.6 of \cite{Viderman13b}.\textcolor{red}{XUe: We may wanna rewrite it or summarize this in Section 3.}

So we get
\[
(1-k \eps)k -O(1/N) \le 2 \eps k + (1-2\eps)x.
\]
So it becomes
\[
(1-2 \eps)k - \eps k^2 \le (1-2\eps)x + O(1/N).
\]
Let $k_0 = \frac{1-2 \eps}{2 \eps}$. Since $\eps \leq 1/4$,  $k_0 \geq 1$.
Suppose  $k$ reaches $k_0 $, which maximizes the left hand side to be $ \frac{(1-2\eps)^2}{4 \eps}$. 
But when $x <  \frac{1-2\eps}{4 \eps} - O(1/N)$  the right hand side is less than $ \frac{(1-2\eps)^2}{4 \eps}$. 
So $k$ can not reach $k_0$.

\end{proof}

%This argument needs $k_0 \ge 1$ and $x\le 1$, which means $\eps \in [1/6,1/4]$.


\begin{theorem}

Let $\Gamma$ be a $(\alpha N, (1-\eps) D_L)$ expander with $\eps \in [1/6, 1/4] $.  The expander code defined by $\Gamma$ has an efficient decoding algorithm with decoding radius $(\frac{1-2\eps}{4\eps})\alpha N - O(1)$.

\end{theorem}
The whole decoding algorithm is as follows.
\begin{algorithm}[h]
\caption{Fixed Find and Decode}\label{alg:FixedFindAndDecode}
\begin{algorithmic}[1]
\Function{FixedFindAndDecode}{$C \in \mathbf{F}_2^N$}
\State $L \gets $ \Call{Find}{$C, \eps$}
\State Apply Theorem \ref{thm:vidermandecfromerasures} with $L$ and $C$ to get a codeword $C'$.
\State \Return $C$
\EndFunction
\end{algorithmic}
\end{algorithm}
\begin{proof}
Let $C$ be a corrupted codeword. 
Let $F$ be the set of errors.
We run Algorithm \ref{alg:FixedFindAndDecode} on $C$.
As $\eps \geq 1/6$,  $\frac{1-2\eps}{4 \eps} \leq 1$. 
Thus by Claim \ref{claim:errors_in_L}, $F$ is contained in $L$ after finding erasures.
As $|F| = x\alpha N \leq \frac{1-2\eps}{4\eps}\alpha N - O(1)$ and $\eps \leq 1/4$, by Claim \ref{claim:bound_L}, $L$ has size at most $k_0 \alpha N = \frac{1-2 \eps}{2 \eps}\alpha N $, which is at least $\alpha N$, since $\eps \leq 1/4$.
Notice that $\Gamma$ is an $(\alpha N, (1-\eps) D)$ expander, and $1-k_0\eps-O(1/N)>1/2$.
Hence by Theorem \ref{thm:decfromerasures}, we can regard $C$ as having erasures in $L$ and then decode from these erasures.
\end{proof}










\subsection{Guess threshold for the case $\eps \leq 1/6$}






Consider the expander code on an $(\alpha N, (1-\eps)D)$ bipartite expander $\Gamma$. We provide an efficient algorithm to decode more errors in this section by guessing the expansion of the corrupted set. 

%For ease of exposition, we only consider $\eps \le 1/6$ in this section. 
We describe our algorithm in Algorithm~\ref{alg:decoding_small_eps}.

\begin{algorithm}[h]
\caption{Decoding Algorithm for $\eps\le 1/6$}\label{alg:decoding_small_eps}
\begin{algorithmic}[1]
\Function{Decoding}{$C \in \mathbf{F}_2^N$ }
	\For {all possible size $x \alpha N$ of $F$}
	\For {all possible expansion $(1-\gamma) \cdot D |F|$}
	    \If{$\gamma x \ge \eps$}
	        \State $\Delta \gets \sqrt{\gamma x \eps}$
	    \Else
	        \State $\Delta  \gets \eps$
	    \EndIf
	    \State $C' \gets $ \Call{Find}{$C \in \mathbf{F}_2^n$ and $\Delta$}
	    \State \Return $C'$ if $d(C,C')\le \frac{\alpha}{4 \eps} N$
	\EndFor
    \EndFor
\EndFunction
%\Function{Find}{$C \in \mathbf{F}_2^n$ and $\Delta$}
%\State $L \gets \emptyset$ 
%\State $R \gets \{\text{wrong parity checks of } C\}$
%\While{$\exists i\notin L$ s.t. $|\Gamma(i) \cap R| \ge (1-2\Delta)D$}
%\State $L \gets L \cup \{i\}$
%\State $R \gets R \cup \Gamma(i)$
%\EndWhile
%\State Apply the erasure decoding algorithm in Theorem \ref{thm:vidermandecfromerasures}, on input $L$ and $C$, to return a codeword $C'$.
%\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:guessexpansion}
Consider the expander code defined by an $(\alpha N, (1-\eps)D)$ expander.
For $\eps< \frac{3-2\sqrt{2}}{2}$, Algorithm~\ref{alg:decoding_small_eps} is a decoding algorithm which corrects  at least $\frac{\sqrt{2}-1}{2\epsilon} \alpha N $ errors. 
Next for $\eps \in [\frac{3-2\sqrt{2}}{2}, 1/6]$, 
Algorithm~\ref{alg:decoding_small_eps}   corrects at least $\frac{1-2\eps}{4\eps} \alpha N - O(1)$ errors.

\end{theorem}
 

\textcolor{red}{Remark: (1) I am hiding some small terms in $O(1)$. (2) I did not try to optimize the running time at this moment.}

\begin{proof}

We prove the correctness of Algorithm~\ref{alg:decoding_small_eps} in the rest of this section. Again $F$ always denotes the subset of entries that are flipped by the adversary. Since we enumerate both $x$ for $|F|=x \alpha N$ and $\gamma$ for $\Gamma(F)=(1-\gamma)D|F|$ over all possible values, we assume $x \alpha N$ denotes the correct size of $F$ and $\gamma$ denotes the correct expansion of $F$ such that $\Gamma(F)=(1-\gamma) \cdot D |F|$ in the analysis. 
%So $x < \frac{\sqrt{2}-1}{2\eps}$ and $\gamma \le x \cdot \eps$ for any $x > 1$.

First of all, we bound the expansion of all subsets in $F$.
\begin{claim}\label{clm:worst_expansion}
For any $F$ with $|F|=x \alpha N$ and $|\Gamma(F)|=(1-\gamma) \cdot D |F|$, our choice of $\Delta$ always satisfies that
\[
\forall F' \subseteq F, |\Gamma(F')| \ge (1-\Delta) \cdot D |F'|.
\]
\end{claim}
\begin{proof}
Let $F'$ be the subset of $F$ with the worst expansion, say $|F'|=x' \cdot \alpha N$ and $|\Gamma(F')|=(1-\gamma')D \cdot |F'|$. 

If $x' \le 1$, $|\Gamma(F')| \ge (1-\eps) \cdot D |F'|$ by the property of $\Gamma$. 
This is at least $(1-\Delta)D|F'|$ since $\Delta$ is always at least $\eps$ in the algorithm.

Otherwise, we consider the collisions in $\Gamma(F)$ and $\Gamma(F')$. Since $F'$ is a subset of $F$ of size $x' \cdot \alpha N$, $|\Gamma(F')| \ge (1-x' \cdot \eps) D \cdot x' \alpha N - O(1)$. So we have
\[
x' \alpha N \cdot (x' \cdot \eps) + O(1) \le |F| \cdot \gamma,
\]
because a collision  in $\Gamma(F')$ is also a collision in $\Gamma(F)$. 
This implies $x' \cdot \eps \le \sqrt{\eps x \gamma} = \Delta$ and hence shows the claim.
\end{proof}

Given the guarantee in Claim~\ref{clm:worst_expansion}, one could show $L$ covers all the errors.
\begin{claim}
\label{claim:FsubseteqL}
After the while loop in \textsc{Find}, $F\subseteq L$.
\end{claim}
\begin{proof}
Suppose there are $F\backslash L = B \neq \emptyset$. 
Since $B\subseteq F$, by Claim \ref{clm:worst_expansion}, $|\Gamma(B)| \geq (1-\Delta)D|B|$.
So the number of unique neighbors is at least $(1-2\Delta)D|B|$.
Hence there is a $v\in B$ which has at least $(1-2\Delta)D$ unique neighbors.
But $v$ is not in $L$, meaning it has $<(1-2\Delta)D$ neighbors in $R$.
So it has a unique neighbor which is not in $R$.
This is a contradiction since this unique neighbor corresponds to an unsatisfied check which has to be in $R_0 \subseteq R$. 
\end{proof}

Then we calculate the decoding radii and the size of $L$. 



\begin{claim}\label{clm:upper_bound_neighbors}
For either $\Delta=\eps$ or $\sqrt{\eps \gamma x}$, $|\Gamma(L)| \le |\Gamma(F)| + 2 \Delta D \cdot |L \setminus F|$.
\end{claim}
\begin{proof}
Let $(v_1,\ldots,v_{|L|})$ be the sequence of vertices added to $L$ in the while. By Lemma \ref{lemma:L'allsame}, we can adjust the order of the sequence by putting the vertices in $F$ at first and then put the vertices in $L \setminus F$ after them. The upper bound follows from the fact $F \subseteq L$ from Claim \ref{claim:FsubseteqL} and each vertex in $L \setminus F$ contributes at most $2 \Delta$ to $R$. 
\end{proof}

\begin{claim}
\label{claim:guessExpansionLbound1}
For $\Delta=\sqrt{\eps \gamma x}$, $|L| < \frac{1-2\Delta}{2\eps} \alpha N$.
\end{claim}
\begin{proof}
Suppose $L \ge \frac{1-2\Delta}{2\eps} \alpha N$.
Let $\delta=\frac{1 - 2 \Delta}{2 \eps} - x$.
Consider $L' \subseteq L$ that is constituted by $F$ and the first $\delta \alpha N$ vertices in $L\setminus F$ added in  the while loop. 
So $|L'| = \frac{1-2\Delta}{2\eps} \alpha N$.
From Claim~\ref{clm:upper_bound_neighbors}, $|\Gamma(L')| \le |\Gamma(F)|+2\Delta D\cdot \delta \alpha N$. On the other hand, Lemma~\ref{lem:expansion_larger} implies $|\Gamma(L')| \ge (1-(x+\delta)\eps)D \cdot (x+\delta)\alpha N - O(1)$. Thus we have
\[
(1-(x+\delta)\eps) \cdot (x+\delta)\alpha N - O(1)\le (1-\gamma)x \alpha N + 2 \sqrt{\eps \gamma x} \cdot \delta \alpha N.
\]
In the rest of this proof, we show that our choice of $\delta$ yields
\begin{equation}\label{eq:ineq1}
(1 - (x+\delta)\eps) \cdot (x+ \delta) - O(1/N) > (1-\gamma) x + 2 \sqrt{\eps \gamma x} \cdot \delta.
\end{equation}
This is contradicted to the above discussion. We rewrite  inequality~\eqref{eq:ineq1} as
\[
0 > \eps \delta^2 + (2 \eps x - 1 + 2 \sqrt{\eps \gamma x})\delta + \eps x^2 - \gamma x +  O(1/N) .
\]
When $(2 \eps x - 1 + 2 \sqrt{\eps \gamma x})^2 - 4 \eps \left( \eps x^2 -\gamma x +  O(1/N)  \right)>0$, the quadratic polynomial will be negative at $\delta=\frac{1 - 2 \eps x - 2 \sqrt{\eps \gamma x}}{2\eps}$. To verify $(2 \eps x - 1 + 2 \sqrt{\eps \gamma x})^2 - 4 \eps \left( \eps x^2 -\gamma x +  O(1/N)  \right)>0$, we set $c=\eps x$ to rewrite it as
\[
(2c - 1 + 2 \sqrt{\gamma c})^2 - 4 c^2 + 4 \gamma c -  O(1/N) >0.
\]
This is equivalent to
\[
8 \gamma c + (8c -4 ) \sqrt{\gamma c} + 1 - 4c  - O(1/N) > 0 \Rightarrow 8(\sqrt{\gamma c} +\frac{2c-1}{4})^2  - O(1/N) + 1 - 4c - 8(\frac{2c-1}{4})^2 > 0.
\]
\textcolor{red}{Xue: We may wanna handle the extra $O(1/N)$ term here. At least, we need to change $\leq$ to $<$.}
When $c=\eps x \leq \frac{\sqrt{2}-1}{2}$, i.e. $x \leq \frac{\sqrt{2}-1}{2\eps}$, the residue $1 - 4c - 8(\frac{2c-1}{4})^2 \geq 0$.
So the inequality holds.
\end{proof}

\begin{claim}
\label{claim:guessExpansionLbound2}
For $\Delta=\eps$, $|L| < \frac{1-2\eps}{2\eps} \alpha N$.
\end{claim}
%\textcolor{red}{This proof assumes $x+\delta \ge 1$. But one can bound the case $x+\delta \le 1$ by a similar argument.}
\begin{proof}
%We first assume   $x+\delta \ge 1$.
Suppose $|L| \geq \frac{1-2\eps}{2\eps} \alpha N$.
Consider $L'\subseteq L$ with $|L'| =  \frac{1-2\eps}{2\eps} \alpha N$.
Let $\delta = \frac{1-2\eps}{2\eps} - x$. 
Notice that $\delta >0$ since we only need to consider every $x\leq \frac{1-2\eps}{4\eps} - O(1)$.
We have
\[
(1-(x+\delta)\eps) \cdot (x+\delta) - O(1/N) \le x + 2 \eps \delta.
\]
So this is equivalent to
\[
(1- 2\eps - \eps (x+\delta))(x+\delta)  - O(1/N)  \le (1-2\eps) x
\]
The L.H.S. is maximized at $\delta+x=\frac{1 -2 \eps}{2\eps}$. To get a contradiction, we need to guarantee
\[
(1-2\eps) x < (1-2\eps)^2/4\eps - O(1/N).
\]
Namely $x < \frac{1-2\eps}{4\eps} - O(1/N)$.


%If $x + \delta < 1$, then because $\eps \leq 1/6 < 1/4$, we have $\frac{1-2\eps}{2\eps} \geq 1 > x+ \delta = |L|$.

\end{proof}
Consider we run  Algorithm \ref{alg:decoding_small_eps}.
If $\eps < \frac{3-2\sqrt{2}}{2} $, then by Claim \ref{claim:guessExpansionLbound1} and Claim \ref{claim:guessExpansionLbound2}, when $x \leq  \frac{\sqrt{2}-1}{2\eps}$, we have $|L| < \frac{1-2\eps}{2\eps}\alpha N  $.
If $\eps \in [\frac{3-2\sqrt{2}}{2}, 1/6]$, then again by Claim \ref{claim:guessExpansionLbound1} and Claim \ref{claim:guessExpansionLbound2}, when 
$x <   \frac{1-2\eps}{4\eps} - O(1/N)$, we have $|L| < \frac{1-2\eps}{2\eps} \alpha N$.
Since the expander is an $(\alpha N, (1-\eps)D)$ expander, by Lemma \ref{lem:expansion_larger}, it is also a $(\frac{1-2\eps}{2\eps}\alpha N, \left(\frac{1}{2} + \eps \right) D  - O(1/N)  )$ expander.
Then by Theorem \ref{thm:vidermandecfromerasures}, one can correct all the errors efficiently using $L$ (as the erasure area) and the corrupted codeword, since are the errors are in $L$ by Claim \ref{claim:FsubseteqL}.

\end{proof}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Adaptive thresholds and Flipping}
We consider $\eps \in (1/6,1/4)$ in this section. The basic idea is to guess the expansion $(1-\gamma)$ of the corrupted entries and flip all entries with more than $(1-3\gamma)D_L$ wrong parity checks. 

We describe our algorithm in Algorithm~\ref{alg:decoding_large_eps}. We remark that the flipping only helps us when $1-3\gamma>1-2\eps$. So there are two cases in the decoding procedure. Then we state our main result of this section.
\begin{algorithm}[h]
\caption{Decoding Algorithm for $\eps<1/4$}\label{alg:decoding_large_eps}
\begin{algorithmic}[1]
\Function{Decoding}{$C_0 \in \mathbf{F}_2^n$ and $\gamma_i\in \mathbf{R}, i\in [l]$}
    \State $C \gets C_0$
    \State Set a parameter $c \gets 3$. \textcolor{red}{We may adjust this one to get a better bound}
 \While{$C$ is not a codeword}
    \State Let $F$ be the subset of corrupted entries and assume $\gamma = \gamma_i$ to be its expansion, i.e., $|\Gamma(F)|=(1-\gamma)D \cdot |F|$. 
    \textcolor{red}{We shall enumerate this for a formal algorithm.}   
    \If{$\gamma \ge 2\eps/3$}
     \State $C' \gets$ \Call{FixedFindAndDecode}{$C$}
     \State \Return $C'$
    \Else
    \State Let $L_0$ denote all variables with at least $(1-c \gamma)$ wrong parity checkes
        \State Flip $L_0$ in $C$
    \EndIf
\EndWhile
    \State \Return $C$
\EndFunction
%\Function{FixedFind}{$C \in \mathbf{F}_2^n$}
%\State $L \gets \emptyset$ 
%\State $R \gets \{\text{wrong parity checks of } C\}$
%\While{$\exists i\notin L$ s.t. $|\Gamma(i) \cap R| \ge (1-2\eps)D$}
%\State $L \gets L \cup \{i\}$
%\State $R \gets R \cup \Gamma(i)$
%\EndWhile
%\State $L \gets $ \Call{Find}{$C, \eps$}
%\State Apply Theorem \ref{thm:vidermandecfromerasures} with $L$ and $C$ to return a codeword $C'$.
%\EndFunction
\Function{Final Decoding}{$C_0 \in \mathbf{F}_2^n$}
 \State Enumerate $\gamma_1, \gamma_2, \ldots, \gamma_l$ where $l = c_1 \log N$, with a large enough constant $c_1$.
    \For{enumeration $\gamma_1, \gamma_2, \ldots, \gamma_l$}
        \State $C' \gets$ \Call{Decoding}{$C_0,  \gamma_i, i\in [l]$} 
        \If{$C'$ is a valid codeword}
        \State \Return $C'$
        \EndIf
    \EndFor
\EndFunction
\end{algorithmic}
\end{algorithm}



\begin{theorem}
For any constant $\eps<1/4$, Algorithm~\ref{alg:decoding_large_eps} corrects $(1-\eps-o(1)) \cdot \alpha N$ errors.
\end{theorem}


First of all, we show Function \textsc{FixedFindAndDecode} will recover the codeword whenever $\gamma$ is large.

\begin{claim}\label{clm:small_gamma}
Suppose the subset $F$ of flipped entries has size at most $(1-\eps) \cdot \alpha N$ and its expansion parameter $\gamma \ge \frac{2\eps}{3}$. Then Function \textsc{FixedFindAndDecode} will return a valid codeword.
\end{claim}
\begin{proof}
We prove that $L$ after \textsc{Find} has size at most $\alpha N$. 
Suppose not.
By Lemma \ref{lemma:all_errors_in_L}, we know, after \textsc{Find}, $L$ covers all the errors.
Consider the moment $|L|=\alpha N$. 
Without loss of generality, we assume $F \subseteq L$ (otherwise we can adjust the order of vertices added to $L$ by Lemma \ref{lemma:L'allsame}).

Then we have
\[
(1-\eps) D \alpha N \le | \Gamma(L) | \le  (1-\gamma)D \cdot |F| + 2 \eps D (\alpha N - |F|).
\]
Because the expansion of $F$ is $(1-\gamma)D \cdot |F|$ and when adding any vertex in $L\setminus F$ to $L$, $R$ increases by at most $2\eps D$.
So
\[
(1-\eps) \alpha N \le (1-\gamma) \cdot |F| + 2 \eps (\alpha N - |F|).
\]
This implies $|F| \ge \frac{1-3\eps}{1-\gamma - 2 \eps} \cdot \alpha N$, which is at least  $\frac{1-3\eps}{1-8\eps/3} \alpha N$ given $\gamma \ge 2\eps/3$. Thus, it is contradicted to the assumption of $F \le (1-\eps) \alpha N$ and $\eps<1/4$.
\end{proof}

We know in one of the parallel procedures, $\gamma_i, i\in [l]$ correspond to the correct guesses of the expansions used in the iterations of the Decoding function. 
For this enumeration, we have the following.
\begin{claim}\label{clm:large_gamma}
Suppose $F$ is of size at most $(1-\eps) \alpha N$ and of expansion $\gamma <\frac{2\eps}{3}$. Then flipping $L_0$ will reduce the distance between $C$ and the correct codeword by a small constant fraction.
\end{claim}
\begin{proof}
First of all, $|F \cup L_0| < \alpha N$. To prove it,  we assume $|F \cup L_0|=\alpha N$. So
\[
(1-\eps) \alpha N \le |\Gamma(F \cup L_0)| \le (1-\gamma) |F| + c \gamma \cdot (\alpha N - |F|).
\]
This implies $|F| \ge \frac{1-\eps - c \gamma}{1-\gamma - c \gamma} \cdot \alpha N$, which is minimized at $\gamma=0$. Then we still have $|F| \ge (1-\eps) \alpha N$, contradicted to the assumption.

Next
\begin{equation}\label{eq:F_and_L_0}
   (1-\eps) \cdot D |F \cup L_0| \le \Gamma(F \cup L_0) \le (1-\gamma)|F| + c \gamma |L_0 \setminus F|, 
\end{equation} which gives
\[
(1-\eps-c \gamma)  \cdot |L_0\setminus F| \le (\eps-\gamma) \cdot |F|.
\]

Now we consider $F \setminus L_0$. Each variable in $F \setminus L_0$ contributes at most $(1-c\gamma) D$ unique neighbors. And the total number of unique neighbors is at least $(1-2\gamma)D \cdot |F|$. So the size of $F\setminus L_0$ is at most $2/c \cdot |F|$.

Finally we show 
\[ 
\frac{2}{c} + \frac{\eps -\gamma}{1-\eps - c \gamma}< 1.
\]
For $c=3$, it is equivalent to show
\[
\frac{\eps-\gamma}{1-\eps-3\gamma} < 1/3,
\]
which is always true for $\eps<1/4$. So this implies $|L_0 \setminus F| + |F \setminus L_0|\leq |F|$.
Since $\eps$ is a constant, this means the number of errors is reduced by a small constant fraction.
\end{proof}

 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\section{Adaptive thresholds and Flipping}
We consider $\eps \in (1/6,1/4)$ in this section. The basic idea is to consider two cases about the actual expansion of $F$.

We describe our algorithm in Algorithm~\ref{alg:decoding_large_eps} and state our main result of this section.
\begin{algorithm}[h]
\caption{Decoding Algorithm for $\eps> 1/6$}\label{alg:decoding_large_eps}
\begin{algorithmic}[1]
\Function{Decoding}{$C_0 \in \mathbf{F}_2^n$ and $(\alpha,1-\eps)$}
    \State $C \gets C_0$
    \While{$C$ is not a codeword}
        \State $C' \gets$ \Call{FixedFindAndDecode}{$C$}
        \If{$C'$ is a valid codeword with distance at most $\alpha N$ to $C_0$}
        \State \Return $C'$
        \Else
        \State Let $F$ be the subset of corrupted entries.
        \State Let $\gamma$ be the expansion of $F$, i.e., $|\Gamma(F)|=(1-\gamma)D \cdot |F|$. \textcolor{red}{We shall enumerate this.}
        \State We choose  $c=\frac{(2+o(1))\eps}{\gamma}$, use a threshold $(1- c \gamma)$ to find $L_0$
        \State Flip $L_0$ in $C$
        \EndIf
    \EndWhile
\EndFunction
\Function{FixedFindAndDecode}{$C \in \mathbf{F}_2^n$}
\State $L \gets \emptyset$ 
\State $R \gets \{\text{wrong parity checks of } C\}$
\While{$\exists i\notin L$ s.t. $|\Gamma(i) \cap R| \ge (1-2\eps)D$}
\State $L \gets L \cup \{i\}$
\State $R \gets R \cup \Gamma(i)$
\EndWhile
\State Apply the erasure decoding algorithm in \cite{Viderman13} with $L$ to return a codeword $C'$.
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{theorem}
For any $\delta>0$ and $\eps<1/4$, Algorithm~\ref{alg:decoding_large_eps} corrects $(1-\eps-o(1)) \cdot \alpha N$ errors.
\end{theorem}

First of all, we show Function \textsc{FixedFindAndDecode} will recover the codeword whenever $\gamma$ is large.

\begin{claim}\label{clm:small_gamma}
Suppose the subset $F$ of flipped entries has size at most $(1-\eps) \alpha N$ and its expansion parameter $\gamma \ge \frac{2\eps^2}{1-\eps}$. Then Function \textsc{FixedFindAndDecode} will return a valid codeword.
\end{claim}
\begin{proof}
We prove that $L$ after the while loop has size at most $\alpha N$. Consider the moment $|L|=\alpha N$. Without loss of generality, we assume $F \subseteq L$ (otherwise we adjust the order of vertices added to $L$).

Then we have
\[
(1-\eps) \alpha N \le (1-\gamma) \cdot |F| + 2 \eps (\alpha N - |F|).
\]
This implies $|F| \ge \frac{1-3\eps}{1-\gamma - 2 \eps} \cdot \alpha N$, which is greater than $(1-\eps) \alpha N$ and contradicted to the assumption of $F$.
\end{proof}

\begin{claim}\label{clm:large_gamma}
Suppose the subset $F$ of flipped entries has size at most $(1-\eps) \alpha N$ and its expansion $\gamma <\frac{2\eps^2}{1-\eps}$. Then flipping $L_0$ will reduce the distance between $C$ and the correct codeword.
\end{claim}
\begin{proof}
First of all, $|F \cup L_0| < \alpha N$. To prove it,  we assume $|F \cup L_0|=\alpha N$. So
\[
(1-\eps) \alpha N \le |N(F \cup L_0)| \le (1-\gamma) |F| + c \gamma \cdot (\alpha N - |F|).
\]
This implies $|F| \ge \frac{1-\eps - c \gamma}{1-\gamma - c \gamma} \cdot \alpha N \ge (1-\eps) \cdot \alpha N$ contradicted with our assumption. This shows
\begin{equation}\label{eq:F_and_L_0}
   (1-\eps) \cdot |F \cup L_0| \le (1-\gamma)|F| + c \gamma |L_0 \setminus F|. 
\end{equation}

Now we consider $F \setminus L_0$ and $L_0 \setminus F$. Each variable in $F \setminus L_0$ shares more than $c \gamma$ neighbors with other vertices in $F$. So $N(F \setminus L_0) < (1-c \gamma/2)D \cdot |F \setminus L_0|$ and
 \[
 (1-\gamma)|F| < |F \cap L_0| + (1-c\gamma/2) \cdot |F \setminus L_0| = |F| - c\gamma/2 \cdot |F \setminus L_0|.
 \]
We plug this bound into \eqref{eq:F_and_L_0}:
\[
(1-\eps) |F \cup L_0| \le |F| - c \gamma/2 \cdot |F \setminus L_0| + c \gamma |L_0 \setminus F|.
\]
Namely
\[
c \gamma/2 \cdot |F \setminus L_0| + (1-\eps- c\gamma) |L_0 \setminus F| \le \eps |F|.
\]
So we need $c \gamma/2 > \eps$ and $1-\eps - c \gamma >\eps$ to guarantee that the while loop reduces the number of errors. These require $\eps<1/4$ and $c \gamma>2 \eps$ separately.
\end{proof}
%%%%%%t most $($%%%%%%%%%1-c\gamma/2)D \cdot ||%%%%%%%%%%%at least %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

==> backup2.tex <==

\section{Unique Decoding by Guessing Expansion with Iterative Flipping }\label{sec:guess_flip}
We consider $\eps$ to be an arbitrary constant $ < 1/4 $ in this section.
%\xnote{Why consider $\eps \in (1/6,1/4)$ if Thm 5.1 shows it works for any $\eps < 1/4$?} 
%We follow the notations in Section~\ref{sec:improve_decoding} --- given a string $y$, let $F$ denote the set of corrupted entries and $(1-\gamma)D \cdot |F|$ denote the size of its neighbor set.

We first show an algorithm which has decoding radius $(1-\eps)\alpha N$. 
Then by using Lemma \ref{lem:expansion_larger}, we show that the algorithm achieves decoding radius approximately $\frac{3 \alpha}{16\eps} N$.

The basic idea of the algorithm is to guess the expansion of the corrupted entries in the algorithm, say $(1-\gamma)D$.
Assume we can correctly guess $\gamma$.
For the case $\gamma \geq \frac{2}{3}\eps$, we  do a finding possible corruptions and then decoding from erasures procedure, similar to \cite{Viderman13b}. Because of the case condition, it can be shown that $(1-\eps)\alpha N$ errors can be corrected.
For the case $\gamma < \frac{2}{3}\eps$, we first locate the left subset which contains vertices  having at least $1-3\gamma$ unsatisfied checks. 
We show that this set has (a constant fraction) more corrupted bits than correct bits. 
So we only need to do flipping in this set to reduce the number of errors.
The algorithm iteratively do this to reduce errors significantly and then apply a classic decoding to correct remaining errors.

We describe our algorithm in Algorithm~\ref{alg:decoding_large_eps} and then state our main result of this section.
For ease of exposition, Algorithm~\ref{alg:decoding_large_eps} does exact enumerations, thus it is only a polynomial time algorithm. 
To make it a linear time algorithm we need to do approximate enumerations. See Remark~\ref{remark:EnumerationApprox}.
%\knote{It seems we only need constant number of iterations, because once the number of errors is reduced to e.g. $\alpha N/2$, we can set $h = (1-2\eps)D$ and run one more Find and Decode from erasures to decode the remaining errors. This means we don't need to set $\eta$ then, enumerations can enumerate the exact values.}
%\xnote{Good point. Or we can get linear running time? I guess Algorithm 3 can also be made linear time in this way.}
\begin{algorithm}[H]
\caption{Decoding Algorithm for $\eps<1/4$}\label{alg:decoding_large_eps}\label{alg:MultipleGuessWithFlips}
\begin{algorithmic}[1]


\Function{Final Decoding}{$y \in \mathbf{F}_2^n, \alpha  \in \mathbf{R}, \eps \in \mathbf{R}$} //The main procedure.
 \State Enumerate $\gamma_1, \gamma_2, \ldots, \gamma_l$ where $\ell = O(\frac{1}{1/4-\eps})$.
 For every $ i\in [\ell]$, the enumeration first  enumerate an integer $ a \in [N] $.
 Then  $\gamma_i$ is enumerated by enumerating $b\in [M]$ and taking $\gamma_i$ such that $(1-\gamma_i)D a = b$.
 (This is a polynomial time enumeration. For linear time enumeration, see Remark~\ref{remark:EnumerationApprox})
    \For{enumeration $\gamma_1, \gamma_2, \ldots, \gamma_\ell$}
        \State $C' \gets$ \Call{Decoding}{$y,  \gamma_1, \ldots,\gamma_{\ell}, \alpha, \eps$} 
        \If{$C'$ is a valid codeword  and the distance between $C'$ and $y$ is at most $(1-\eps) \alpha N$} %\xnote{no $D$ here}
        \State \Return $C'$
        \EndIf
    \EndFor
   % \xnote{For this part, is it clear that we can only get one valid codeword? What if we get multiple valid codewords from the enumeration and the function returns with the first one but not the correct one?}
\EndFunction


\Function{Decoding}{$y \in \mathbf{F}_2^n$ and $(\gamma_1,\ldots,\gamma_{\ell}) \in \mathbf{R}^{\ell}, \alpha \in \mathbf{R}, \eps \in \mathbf{R}$}
    \State $z \gets y$
   % \State Set a parameter $c \gets 3$. %\textcolor{red}{We may adjust this one to get a better bound}
   % \State $\gamma_i \gets 1$
 \For{$i=1,\ldots,\ell$}
    %\State Let $F$ be the subset of corrupted entries and assume $\gamma$ to be its expansion, i.e., $|\Gamma(F)|=(1-\gamma)D \cdot |F|$. 
    %\textcolor{red}{We shall enumerate this for a formal algorithm.}   
    \If{$\gamma_i  \ge 2\eps/3 $}
     \State $z \gets$ \Call{FixedFindAndDecode}{$z, \alpha, \eps$} %\textcolor{blue}{Xue: Where is this procedure?}
     \State \Return $z$ 
    \Else
    \State Let $L_0$ denote all variables with at least $(1-3 \gamma_i)$ wrong parity checks
    %\xnote{Why not just use $(1-3 \gamma_i)$?}
        \State Flip $L_0$ in $z$
    \EndIf
\EndFor
    \State Apply the decoding of Theorem \ref{thm:vidermandec} on $z$ and return the result.
     %if the distance between $z$ and $y$ is at most $(1-\eps)D\alpha N$
%    \xnote{This algorithm looks incorret to me. First, we need to initialize $i$ before the while loop and keep changing $i$ inside the loop. Second, for some enumeration of $(r_i)$ we may run out of $r_i$ before the while loop can end. Then what do we do?}
\EndFunction


\Function{FixedFindAndDecode}{$y \in \mathbf{F}_2^N, \alpha \in \mathbf{R}, \eps \in \mathbf{R}$}
\State $L \gets $ \Call{Find}{$y, \eps$}
\State Apply Theorem \ref{thm:decfromerasures} with $L$ and $y$ to get a codeword $C'$.
\State \Return $C'$
\EndFunction% \textcolor{blue}{Why this procedure is here?}


\end{algorithmic}
\end{algorithm}



\begin{theorem}
\label{thm:MultipleGuessWithFlips}
For every small constant $\beta > 0$, for every $\eps \leq 1/4 - \beta $, let $\mathcal{C}$ be an expander code defined by a $(\alpha N, (1-\eps)D)$ expander graph.  There is a linear time decoding algorithm with radius $(1-\eps ) \cdot \alpha N$.


\end{theorem}

\begin{remark}
\label{remark:EnumerationApprox}
In the analysis we consider 
Algorithm \ref{alg:MultipleGuessWithFlips}.
Notice that Algorithm  \ref{alg:MultipleGuessWithFlips} only runs in polynomial time because of the enumeration procedure.
We claim that the running time can be made linear if we replace the whole enumeration procedure by directly enumerating each $\gamma_i$ from the set $\{0, \eta, 2\eta, \ldots, \lceil\frac{1}{\eta} \rceil \eta \}$, where $\eta$ is a small enough constant (compared to $\beta$). 
The same decoding radius holds using this approximate enumeration.
However, for ease of exposition, our analysis is based on algorithm  \ref{alg:MultipleGuessWithFlips}. 
%\textcolor{blue}{Xue:I think we shall mention the enumeration in the 3rd paragraph before ALG 2 to make it clear this is for ease of exposition. Similar comment for Remark 6.2.}
%\textcolor{blue}{Xue: But we also enumerate $a \in [N]$. Why do we need to do this? It would be better to change the function name to ``Main" or something else.}
\end{remark}

%\textcolor{blue}{Xue: We shall state that the running time could be linear! That's the most attractive feature of expander codes.} \xnote{I think we should at least add a comment that the running time can be made linear by sparsifying the enumeration. Same for Theorem~\ref{thm:guessexpansion}}
%\knote{The running time still cannot be linear yet for this algorithm. For Theorem~\ref{thm:guessexpansion} it can be linear, but we may trade in some other parameters since we need enumeration step length $\eta$}
We focus on the $i$-th iteration, and show that we can make progress (reduce the number of errors) in this iteration.
Let $F_i$ denote the set of errors at the beginning of iteration $i$ and $\gamma(F_i) \in [0,\eps]$ be the parameter such that $| \Gamma(F_i) | = (1-\gamma(F_i)) \cdot D|F_i|$. %\xnote{not by $|F_i|$, but by $F_i$.}
%When $i$ is clear from the context we just use $\gamma$ for simplicity of exposition.
%\xnote{The format here is annoying. I guess we assume that a reader has already seen the algorithm, but it's actually on the next page. So when I read here I have no idea what $\eta$, $\gamma_i, i\in [l]$ are referring to.}
%Here $\eta$ is the precision parameter we picked in the algorithm and can be an arbitrary small constant. 
%\textcolor{blue}{Xue: Notataion: (1) Why we use $\beta$ instead of $\beta$? (2) I prefer $(\gamma_1,\ldots,\gamma_{\ell})$ or $(\gamma_i)_{i \in [\ell]}$ to denote the sequence instead of $\gamma_i, i \in [l]$.}

%We know in one of the enumerations, $\gamma_i, i\in [l]$ are exactly the correct expansion parameters, i.e. $\forall i\in [l]$ in the $i$-th iteration,  $\gamma(F_i) = \gamma_i$. \textcolor{blue}{Xue: (1) I think this paragraph shall be moved to the Proof of Theorem 5.1. We will only discuss one iteration before that proof. (2) The definition of $\gamma$ missing some terms.} %\xnote{You mean in ea iteration, a fixed $\gamma$ is always in $[\gamma_i - \eta, \gamma_i]$?}
%So we mainly focus on this enumeration, showing its corresponding procedure can do the correct decoding.

Next, we show Function \textsc{FixedFindAndDecode} will recover the codeword directly whenever $\gamma(F_i)$ is large.

%\textcolor{blue}{Xue: In line 5 of Algorithm 5, we do not know $\gamma$. We shall be more careful about this proof --- how about write Claim 5.2 and 5.3 for just one iteration then defer all discusion about the sequence $(\gamma_i)_{i}$ to the proof of THM 5.1?}



\begin{claim}\label{clm:small_gamma}
When $|F_i| < (1-\eps  ) \cdot \alpha N$, if $\gamma(F_i) \ge \frac{2\eps}{3}$, then Function \textsc{FixedFindAndDecode} will return a valid codeword.
\end{claim}

\begin{proof}
Let $\gamma:= \gamma(F_i)$. We prove that $L$ after \textsc{Find} has size at most $\alpha N$. 
Suppose not.
Since $|F_i| \leq (1-\eps  ) \cdot \alpha N$, for every nonempty $ F'\subseteq F_i,  |\Gamma(F_i)| \geq (1-\eps)D|F'|$, so by Lemma \ref{lemma:all_errors_in_L},   after \textsc{Find}, $L$ covers all the errors. %\xnote{The logic of this sentence is weird. I think the reason we can use Lemma \ref{lemma:all_errors_in_L} is that $|F_i| \leq (1-\eps  ) \cdot \alpha N$, not that $\gamma \ge  \frac{2\eps}{3}$.}
Consider the moment $|L|=\alpha N$. 
Without loss of generality, we assume $F_i \subseteq L$ (otherwise we can adjust the order of vertices added to $L$ by Lemma \ref{lemma:L'allsame}).

Then we have
\[
(1-\eps) D \alpha N \le | \Gamma(L) | \le  (1-\gamma)D \cdot |F_i| + 2 \eps D (\alpha N - |F_i|),
\]
because the expansion of $F_i$ is $(1-\gamma)D \cdot |F_i|$ and when adding any vertex in $L\setminus F_i$ to $L$, $R$ increases by at most $2\eps D$.
So
\[
(1-\eps) \alpha N   \le (1-\gamma) \cdot |F_i| + 2 \eps (\alpha N - |F_i|).
\]

%\xnote{How do we get the above inequality? How can we just replace $|F_i|$ in the LHS by $\alpha N$? In the previous inequality, the LHS should use the expansion of $|L|=\alpha N$ instead of $F_i$.}
As $\gamma  \leq \eps$, $\eps \leq 1/4$, so $1-\gamma - 2 \eps > 0$, hence
this implies $|F_i| \ge \frac{1-3\eps}{1-\gamma - 2 \eps} \cdot \alpha N $. %\xnote{This needs $1-\gamma - 2 \eps > 0$, which may not be true.}
Since $\gamma(F_i) \geq \frac{2\eps}{3} $, we have   $|F_i| \geq \frac{1-3\eps}{1-8\eps/3 } \alpha N  $. 
When  $\eps \leq 1/4$, one can check that $\frac{1-3\eps}{1-8\eps/3 }  \geq 1-\eps   $ always holds.
It is contradicted to the assumption that $F_i \le (1-\eps  ) \alpha N$.

As $L$ after \textsc{Find} has size at most $\alpha N$, the expander is an $(\alpha N, (1-\eps)D)$ expander, with $\eps <1/4-\beta$, by Corollary \ref{thm:decfromerasures}, we can correct all the errors using $L$ and $z$.
\end{proof}

Next we discuss the case that  $\gamma_i=\gamma(F_i)$ is less than $2\eps/3$ in the ELSE branch of the IF. We show that flipping $L_0$ will reduce the number of errors.

\begin{claim}\label{clm:large_gamma}
If $F_i$ is of size smaller than $(1-\eps  ) \alpha N$ and $\gamma_i = \gamma(F_i)$ is less than $\frac{2\eps}{3}$, then flipping $L_0$ will reduce the distance between $z$ and the correct codeword by $\frac{4}{3}\beta$ fraction.
\end{claim}
\begin{proof}
First of all, let $\gamma:=\gamma(F_i)$ and $N':=\frac{|F_i|}{(1-\eps) \alpha}$. We show that $|F_i \cup L_0| < \alpha N'$. 
To prove it,  assume $|F_i \cup L_0|=\alpha N'$, i.e. we only take $\alpha N' - |F_i|$ elements from $L_0\setminus F_i$, consider these elements together with elements in $F_i$.
By the expander property, $(1-\eps)D \alpha N'   \le |\Gamma(F_i \cup L_0)|$.
Also notice that $|\Gamma(F_i)| = (1-\gamma)D |F_i|$ and adding each element of $L_0\setminus F_i$ to $L_0$ contributes at most $3\gamma_i D$ to  $|\Gamma(F_i \cup L_0)|$.
So
\[
(1-\eps)D \alpha N'   \le |\Gamma(F_i \cup L_0)| \le (1-\gamma)D |F_i| + 3 \gamma_i D \cdot (\alpha N' - |F_i|).
\]
%\xnote{Needs some explanation of this inequality, also, why enough to just consider $|F_i \cup L_0|=\alpha N'$}
This implies $|F_i| \ge \frac{1-\eps - 3 \gamma_i}{1-\gamma - 3 \gamma_i} \cdot \alpha N'$.
Again we know $  \gamma_i = \gamma$ and this is minimized when $\gamma  = 0$. %\textcolor{blue}{Xue: We need to handle $\eta_0$. This also needs $(1+3 \eta_0)/(3+1) \ge \eps?$}
Thus  $|F_i| \ge (1-\eps) \alpha N'$, contradicted to the assumption.

Since $|F_i\cup L_0| <\alpha N'$, now again we have
\begin{equation}\label{eq:F_and_L_0}
   (1-\eps) \cdot D |F_i \cup L_0| \le \Gamma(F_i \cup L_0) \le (1-\gamma)D|F_i| + 3 \gamma_i D|L_0 \setminus F_i|.
\end{equation}
As $ |F_i \cup L_0| = |L_0 \setminus F_i| + |F_i| $,  %\textcolor{blue}{Xue: Not from this fact --- we split $F_i \cup L_0$ here}
this gives
\[
(1-\eps-3 \gamma_i)  \cdot |L_0\setminus F_i| \le (\eps-\gamma) \cdot |F_i|.
\]

Now we consider $F_i \setminus L_0$. Each variable in $F_i \setminus L_0$ contributes at most $(1-3\gamma_i) D$ unique neighbors. And the total number of unique neighbors is at least $(1-2\gamma)D \cdot |F_i|$. So the size of $F_i\setminus L_0$ is at most $\frac{2\gamma}{3\gamma_i} \cdot |F_i|$.

Finally we show 
\[ 
\frac{2\gamma}{3\gamma_i}  + \frac{\eps -\gamma}{1-\eps - 3 \gamma_i}< 1 -  O(\beta).
\]
As $\gamma = \gamma_i$,
the L.H.S. is at most
\[
\frac{2  }{3 }  + \frac{\eps - \gamma_i  }{1-\eps - 3 \gamma_i }.
\]
We know  $\eps \leq 1/4 - \beta$ and $\gamma_i \in [0, \frac{2}{3}\eps]$. 
One can check that this is at most  $1- \frac{4}{3}\beta$.
%\textcolor{blue}{My calculation does not show this unless we have $\beta=\Omega(\eta)$.}
%For $3=3$, it is equivalent to show
%\[
%\frac{\eps-\gamma}{1-\eps-3\gamma} < 1/3,
%\]
%which is always true for $\eps<1/4$. So this implies $|L_0 \setminus F_i| + |F_i \setminus L_0|\leq |F_i|$.
%Since $\eps$ is a constant, this means the number of errors is reduced by a small constant fraction.
\end{proof}

\begin{proofof}{Theorem \ref{thm:MultipleGuessWithFlips}}
The decoding algorithm is Algorithm \ref{alg:MultipleGuessWithFlips}.
Given the parameter $\beta$, we first set up a large enough constant $\ell$ based on $\beta$.
Then we apply the algorithm on an input corrupted codeword, using parameter $\ell$. 
The algorithm first do the enumerations.
We know in one of the enumerations, $(\gamma_i)_{i\in [l]}$ provide exactly the correct expansion parameters, i.e. $\forall i\in [l]$ in the $i$-th iteration,  $\gamma(F_i) = \gamma_i$.
Next we consider every iteration.
If $\gamma_i \geq 2\eps/3 $, then by Claim \ref{clm:small_gamma}, the algorithm returns the correct codeword.
If $\gamma_i < 2\eps/3$, then by  Claim \ref{clm:large_gamma}, the number of errors can be reduced by $O(\beta)$ fraction. 
So in the worst case, when $\ell \geq \log_{1-O(\beta)}\frac{1}{3}$, the number of errors can be reduced to at most $\alpha N / 3$.
So finally the algorithm applies the decoding algorithm from Theorem \ref{thm:vidermandec}, which corrects the remaining errors.

The running time of Algorithm \ref{alg:MultipleGuessWithFlips} is polynomial, since $\ell = O(1)$ and our enumeration for $a$ takes $O(N)$ time for each $\gamma_i$ takes $O(M)$ time. Moreover, the algorithm can be modified to be a linear time algorithm, by  enumerating each $\gamma_i$ from the set $\{0, \eta, 2\eta, \ldots, \lceil\frac{1}{\eta} \rceil \eta \}$, where $\eta$ is a small enough constant (comparing to $\beta$). 
One can check that we can get the same parameters by a similar analysis.

\end{proofof}



By using Theorem \ref{thm:MultipleGuessWithFlips} and Lemma \ref{lem:expansion_larger} we can get the following result.
%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{theorem}
For every constant $\beta > 0$, for every $ \eps \leq 1/4 - \beta $, 
if $\mathcal{C}$ is an expander code defined by an $(\alpha N, (1-\eps)D)$ expander,
 then there is a linear time decoding algorithm for $\mathcal{C}$ which has decoding radius $(\frac{3\eps}{16} - O_\eps(\beta))\alpha N$. 
\end{theorem}
\xnote{I think by setting $\beta$ appropriately, we should be able to rewrite the theorem statement as follows. Check it. Also, $\eps$ should be in the denominator.}
%In fact, from the calculation I believe the decoding radius should be $\frac{3\eps}{16}\alpha N -O_{\eps}(1)$.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{thm:MultipleGuessWithFlipsFinal}
For every constants $ \eps \in (0, \frac{1}{4}), \eta>0$, 
if $\mathcal{C}$ is an expander code defined by an $(\alpha N, (1-\eps)D)$ expander,
 then there is a linear time decoding algorithm for $\mathcal{C}$ which has decoding radius $(\frac{3 \alpha}{16 \eps} - \eta) N$. 
\end{theorem}

\begin{algorithm}[H]
\caption{Decoding Algorithm for $\eps<1/4$ for Larger distance}\label{alg:MultipleGuessWithFlipsLarger}
\begin{algorithmic}[1]
\Function{Final Decoding For Large Distance}{$y\in \mathbf{F}_2^N, \alpha \in \mathbf{R}, \eps \in \mathbf{R}$}
\State Let $k = (1/4-\beta - O_\eps(1/N))/\eps$, with $\beta$ being a small enough constant.
\State Let $z \gets$  \Call{Final Decoding}{$y, k\alpha, k \eps + O_\eps(1/N)$} .
\State \Return $z$.
\EndFunction
\end{algorithmic}
\end{algorithm}
%\xnote{What is $\beta$ in the algorithm?}
\begin{proof}
Consider Algorithm \ref{alg:MultipleGuessWithFlipsLarger}.
By Lemma \ref{lem:expansion_larger}, the expander graph is also a $ (k\alpha N, (1-k\eps)D - O_\eps(1/N)) $ expander for $k\geq 1$.
If taking $k$ to be such that $(1-k\eps)D - O_\eps(1/N) \leq 1/4 - \beta$ with $\beta$ small enough, then by Theorem \ref{thm:MultipleGuessWithFlips}, there is a decoding algorithm with radius $(1 - k\eps - O_\eps(1/N))k\alpha N$.
When $k = (1/4-\beta - O_\eps(1/N))/\eps$, this is maximized to be $(\frac{3}{16\eps} - O_{\eps}(\beta))\alpha N$. 
We can take $\beta$ to be small enough such that decoding radius $(\frac{3 \alpha}{16 \eps} - \eta) N$.
The running time is linear by Theorem~\ref{thm:MultipleGuessWithFlips}.
\end{proof}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\section{Adaptive thresholds and Flipping}
We consider $\eps \in (1/6,1/4)$ in this section. The basic idea is to consider two cases about the actual expansion of $F$.

We describe our algorithm in Algorithm~\ref{alg:decoding_large_eps} and state our main result of this section.
\begin{algorithm}[h]
\caption{Decoding Algorithm for $\eps> 1/6$}\label{alg:decoding_large_eps}
\begin{algorithmic}[1]
\Function{Decoding}{$C_0 \in \mathbf{F}_2^n$ and $(\alpha,1-\eps)$}
    \State $C \gets C_0$
    \While{$C$ is not a codeword}
        \State $C' \gets$ \Call{FixedFindAndDecode}{$C$}
        \If{$C'$ is a valid codeword with distance at most $\alpha N$ to $C_0$}
        \State \Return $C'$
        \Else
        \State Let $F$ be the subset of corrupted entries.
        \State Let $\gamma$ be the expansion of $F$, i.e., $|\Gamma(F)|=(1-\gamma)D \cdot |F|$. \textcolor{red}{We shall enumerate this.}
        \State We choose  $c=\frac{(2+o(1))\eps}{\gamma}$, use a threshold $(1- c \gamma)$ to find $L_0$
        \State Flip $L_0$ in $C$
        \EndIf
    \EndWhile
\EndFunction
\Function{FixedFindAndDecode}{$C \in \mathbf{F}_2^n$}
\State $L \gets \emptyset$ 
\State $R \gets \{\text{wrong parity checks of } C\}$
\While{$\exists i\notin L$ s.t. $|\Gamma(i) \cap R| \ge (1-2\eps)D$}
\State $L \gets L \cup \{i\}$
\State $R \gets R \cup \Gamma(i)$
\EndWhile
\State Apply the erasure decoding algorithm in \cite{Viderman13} with $L$ to return a codeword $C'$.
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{theorem}
For any $\delta>0$ and $\eps<1/4$, Algorithm~\ref{alg:decoding_large_eps} corrects $(1-\eps-o(1)) \cdot \alpha N$ errors.
\end{theorem}

First of all, we show Function \textsc{FixedFindAndDecode} will recover the codeword whenever $\gamma$ is large.

\begin{claim}\label{clm:small_gamma}
Suppose the subset $F$ of flipped entries has size at most $(1-\eps) \alpha N$ and its expansion parameter $\gamma \ge \frac{2\eps^2}{1-\eps}$. Then Function \textsc{FixedFindAndDecode} will return a valid codeword.
\end{claim}
\begin{proof}
We prove that $L$ after the while loop has size at most $\alpha N$. Consider the moment $|L|=\alpha N$. Without loss of generality, we assume $F \subseteq L$ (otherwise we adjust the order of vertices added to $L$).

Then we have
\[
(1-\eps) \alpha N \le (1-\gamma) \cdot |F| + 2 \eps (\alpha N - |F|).
\]
This implies $|F| \ge \frac{1-3\eps}{1-\gamma - 2 \eps} \cdot \alpha N$, which is greater than $(1-\eps) \alpha N$ and contradicted to the assumption of $F$.
\end{proof}

\begin{claim}\label{clm:large_gamma}
Suppose the subset $F$ of flipped entries has size at most $(1-\eps) \alpha N$ and its expansion $\gamma <\frac{2\eps^2}{1-\eps}$. Then flipping $L_0$ will reduce the distance between $C$ and the correct codeword.
\end{claim}
\begin{proof}
First of all, $|F \cup L_0| < \alpha N$. To prove it,  we assume $|F \cup L_0|=\alpha N$. So
\[
(1-\eps) \alpha N \le |N(F \cup L_0)| \le (1-\gamma) |F| + c \gamma \cdot (\alpha N - |F|).
\]
This implies $|F| \ge \frac{1-\eps - c \gamma}{1-\gamma - c \gamma} \cdot \alpha N \ge (1-\eps) \cdot \alpha N$ contradicted with our assumption. This shows
\begin{equation}\label{eq:F_and_L_0}
   (1-\eps) \cdot |F \cup L_0| \le (1-\gamma)|F| + c \gamma |L_0 \setminus F|. 
\end{equation}

Now we consider $F \setminus L_0$ and $L_0 \setminus F$. Each variable in $F \setminus L_0$ shares more than $c \gamma$ neighbors with other vertices in $F$. So $N(F \setminus L_0) < (1-c \gamma/2)D \cdot |F \setminus L_0|$ and
 \[
 (1-\gamma)|F| < |F \cap L_0| + (1-c\gamma/2) \cdot |F \setminus L_0| = |F| - c\gamma/2 \cdot |F \setminus L_0|.
 \]
We plug this bound into \eqref{eq:F_and_L_0}:
\[
(1-\eps) |F \cup L_0| \le |F| - c \gamma/2 \cdot |F \setminus L_0| + c \gamma |L_0 \setminus F|.
\]
Namely
\[
c \gamma/2 \cdot |F \setminus L_0| + (1-\eps- c\gamma) |L_0 \setminus F| \le \eps |F|.
\]
So we need $c \gamma/2 > \eps$ and $1-\eps - c \gamma >\eps$ to guarantee that the while loop reduces the number of errors. These require $\eps<1/4$ and $c \gamma>2 \eps$ separately.
\end{proof}
%%%%%%t most $($%%%%%%%%%1-c\gamma/2)D \cdot ||%%%%%%%%%%%at least %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

==> backup3.tex <==
\section{Improved Unique Decoding  for  $\eps \leq 1/8$}\label{sec:improve_decoding}

 


Consider the expander code on an $(\alpha N, (1-\eps)D)$ bipartite expander $G$. 
For the case of $\eps \le 1/8$ we provide an efficient algorithm,  i.e. Algorithm~\ref{alg:decoding_small_eps}, to decode more errors.
It is again by guessing the expansion of the corrupted entries. 
For easy of exposition, Algorithm~\ref{alg:decoding_large_eps} does exact enumerations when guessing parameters, thus it only runs in polynomial time.
To make it a linear time algorithm we need to do approximate enumerations instead. See Remark~\ref{remark:EnumerationApproximate2}.


\begin{algorithm}[H]
\caption{Decoding Algorithm for $\eps\le 1/8$}\label{alg:decoding_small_eps}
\begin{algorithmic}[1]
\Function{Decoding}{$y \in \mathbf{F}_2^N$ }
	\For {every integer $i \in [1, N]$, let $x$ satisfy $x \alpha N = i$} 
	\For {every integer $j \in [1, M]$, let $\gamma$ satisfy $(1-\gamma) \cdot D \cdot i = j $}
	%\xnote{I find these sentences confusing. Specifically, what does ``all possible size" of $F$ mean? Which sizes are possible, according to what? The correct way to write should be: (e.g.), for all integers $y \in [0, N]$, let $|F|=x \alpha N=y$, for all integers $z \in [0, M]$, let $\Gamma(F)=(1-\gamma) \cdot D |F|=z$.}
	\\(For easy of exposition we do exact enumerations. For linear time algorithm, see Remark~\ref{remark:EnumerationApproximate2}.)
	    \If{$\gamma x \ge \eps$ and $x\geq 1$}
	        \State $\Delta \gets \sqrt{\gamma x \eps} + \frac{c}{N}$ with $c:=c(\eps)$ being a large enough constant.
	    \Else
	        \State $\Delta  \gets \eps$
	    \EndIf
	    \State $L \gets $ \Call{Find}{$y \in \mathbf{F}_2^n$ and $\Delta$}
	    \State Apply Theorem \ref{thm:decfromerasures} with $L$ and $y$ to get a codeword $C'$.
	    \State \Return $C'$ if distance between $C'$ and $y$ is $\le \frac{1-2\eps}{4 \eps}\alpha N $ where the distance comes from Theorem~\ref{thm:dist_expander}.
	  %  \xnote{Is this enough? $\frac{\alpha N}{4 \eps}$ may actually be slightly larger than half distance.}
	\EndFor
    \EndFor
\EndFunction
%\Function{Find}{$C \in \mathbf{F}_2^n$ and $\Delta$}
%\State $L \gets \emptyset$ 
%\State $R \gets \{\text{wrong parity checks of } C\}$
%\While{$\exists i\notin L$ s.t. $|\Gamma(i) \cap R| \ge (1-2\Delta)D$}
%\State $L \gets L \cup \{i\}$
%\State $R \gets R \cup \Gamma(i)$
%\EndWhile
%\State Apply the erasure decoding algorithm in Theorem \ref{thm:vidermandecfromerasures}, on input $L$ and $C$, to return a codeword $C'$.
%\EndFunction

\end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:guessexpansion}
Consider the expander code defined by an $(\alpha N, (1-\eps)D)$ expander.
For $\eps< \frac{3-2\sqrt{2}}{2}$, there is a linear time decoding algorithm with  radius $\frac{\sqrt{2}-1}{2\epsilon} \alpha N -O_{\eps}(1) $. 
Next for $\eps \in [\frac{3-2\sqrt{2}}{2}, 1/8]$, 
there is a linear time decoding algorithm with   radius $\frac{1-2\eps}{4\eps} \alpha N - O_{\eps}(1)$.

\end{theorem}

\begin{remark}
\label{remark:EnumerationApproximate2}
In Algorithm \ref{alg:decoding_small_eps} we do exact enumerations for $x$ and $\gamma$, for ease of exposition and analysis.
The running time of Algorithm \ref{alg:decoding_small_eps} is polynomial instead of linear.
However, the algorithm can be modified to be in linear time if we enumerate $x$ and  $\gamma$ from the set $\{0, \eta, 2\eta, \ldots, \lceil\frac{1}{\eta} \rceil \eta \}$, where $\eta$ is a small   constant.
The same decoding radius holds using this approximate enumeration.
%The decoding radii will loose $O(\eta)$, but as long as   $\eta$ is small enough, they can be absorbed by the $O_\eps(1)$ terms.
%\textcolor{blue}{Xue: I guess $\gamma$ means $j$, what about $i$? Shall mention the decoding radius will lose $O(\eta)$.}\xnote{Will the $O(\eta)$ loss be in the coefficient of $\alpha N$ or not?}
\end{remark}

%\knote{it seems we can show for every $\eps \leq 1/4$, if taking $h = (1-2\eps)D$, decoding radius can be $\frac{1-2\eps}{4\eps}$. This is better than the above theorem when $\eps = 1/100$ e.g.}\xnote{Really? That would be nice since it approaches the half distance bound when $\eps \to 0$. However I'm a little skeptical.}
%\xnote{We should try to unify statements in theorems. For example, here the theorem uses ``corrects at least ... errors", while in the previous section the theorem uses ``with decoding radius..." } 

%\textcolor{red}{Remark: (1) I am hiding some small terms in $O(1)$. (2) I did not try to optimize the running time at this moment.}
%\xnote{Again, are we using Thm 1.3or Thm 2.6? What does $d(C, C')$ mean? For a decoding algorithm is it enough to just return a codeword ?}
 

We prove the correctness of Algorithm~\ref{alg:decoding_small_eps} in the rest of this section. Again $F$ always denotes the subset of entries that are flipped by the adversary. Since we enumerate both $x \alpha N = i$   and $(1-\gamma)D x\alpha N = j$  over all possible values. 
One pair of them correspond to  the correct size of $F$, i.e. $|F| = x \alpha N$ and   the correct expansion size of $F$ i.e. $|\Gamma(F)|=(1-\gamma) \cdot D |F|$.
Now we only consider this pair $x$ and $\gamma$  in the following analysis.
%So $x < \frac{\sqrt{2}-1}{2\eps}$ and $\gamma \le x \cdot \eps$ for any $x > 1$.
%\textcolor{blue}{Xue: Maybe it is better to use ``assume" or ``pretend" in Algorithm 3 instead of ``let". $F$ and $\Gamma(F)$ are out of our control.}

First of all, we bound the expansion of all subsets in $F$.
\begin{claim}\label{clm:worst_expansion}
%For any $F$ with $|F|=x \alpha N$ and $|\Gamma(F)|=(1-\gamma) \cdot D |F|$, 
Our choice of $\Delta$ always satisfies that
\[
\forall F' \subseteq F, |\Gamma(F')| \ge (1-\Delta) \cdot D |F'|.
\]
\end{claim}
\begin{proof}
Let $F'$ be the subset of $F$ with the worst expansion and denote $|F'| = x' \cdot \alpha N$. %and $|\Gamma(F')|=(1-\gamma')D \cdot |F'|$. \xnote{$\gamma'$ never used later?}

If $x' \le 1$, $|\Gamma(F')| \ge (1-\eps) \cdot D |F'|$ by the expansion property of the expander. 
This is at least $(1-\Delta)D|F'|$ since $\Delta$ is always at least $\eps$ in the algorithm.

Otherwise, we consider the collisions   in $\Gamma(F)$ and $\Gamma(F')$.%\xnote{Have we defined ``collisions" before?}
~By collision we mean that given an arbitrary order of the edges, if one edge in this order has its right ending the same as any other edge in previous of it, then this is called a collision. 
Since $F'$ is  of size $x' \cdot \alpha N$, by Lemma \ref{lem:expansion_larger}, $|\Gamma(F')| \ge (1-x' \cdot \eps) D \cdot x' \alpha N - O_\eps(1)$. So we have that the total number of collisions for edges with left endings in $F'$ is at most the total number of collisions for edges with left endings in $F$, because a collision  in $\Gamma(F')$ is also a collision in $\Gamma(F)$, according to an arbitrary order of all edges connected to vertices in $F$. 
So
\[
x' \alpha N \cdot (x' \cdot \eps)D  + O_\eps(1) \le |F| \cdot \gamma D.
\]
This implies $x' \cdot \eps \le \sqrt{\gamma x\eps } = \Delta - \frac{c}{N}$ and hence $|\Gamma(F')| \ge (1-\Delta+\frac{c}{N}) D \cdot |F'| - O_\eps(1) \geq  (1-\Delta) D \cdot |F'|$, when $c$ is large enough.
%\xnote{There is a problem here. From $x' \cdot \eps \le \sqrt{\eps x \gamma} = \Delta$ we can only get $|\Gamma(F')| \ge (1-\Delta) D \cdot |F'| - O(1)$.}
\end{proof}

Given the guarantee in Claim~\ref{clm:worst_expansion}, one can show that $L$ contains all the errors.
%\textcolor{blue}{Xue: Clarify what we mean ``correct"?}
\begin{claim}
\label{claim:FsubseteqL}
After step 9 in Algorithm~\ref{alg:decoding_small_eps}, we have $F\subseteq L$.
\end{claim}

\begin{proof}
By Claim \ref{clm:worst_expansion}, $\forall F' \subseteq F, |\Gamma(F')| \ge (1-\Delta) \cdot D |F'|$.
So $\forall F' \subseteq F, |\Gamma^1(F')| \ge (1-2\Delta) \cdot D |F'|$.
By Lemma \ref{lemma:all_errors_in_L}, we know $F\subseteq L$ after \textsc{Find}.
\end{proof}

%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}
Suppose there are $F\setminus L = B \neq \emptyset$. 
Since $B\subseteq F$, by Claim \ref{clm:worst_expansion}, $|\Gamma(B)| \geq (1-\Delta)D|B|$.
So the number of unique neighbors is at least $(1-2\Delta)D|B|$.
Hence there is a $v\in B$ which has at least $(1-2\Delta)D$ unique neighbors.
But $v$ is not in $L$, meaning it has $<(1-2\Delta)D$ neighbors in $R$.
So it has a unique neighbor which is not in $R$.
This is a contradiction since this unique neighbor corresponds to an unsatisfied check which has to be in $R_0 \subseteq R$. 
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%
Then we calculate the decoding radius and the size of $L$. 


%%%%%%%%%%%%%%%%%%% The following claim seems a bit unflexible to use because when we need it usually we already argued that L is generated by first adding $F$ then other vertices. Also it can only work for those moments where |L| \geq |F| 
\iffalse
\begin{claim}\label{clm:upper_bound_neighbors}
For both $\Delta=\eps$ and $\Delta=\sqrt{\eps \gamma x}$, $|\Gamma(L)| \le |\Gamma(F)| + 2 \Delta D \cdot |L \setminus F|$.
\end{claim}
\begin{proof}
Let $(v_1,\ldots,v_{|L|})$ be the sequence of vertices added to $L$ in the while. By Lemma \ref{lemma:L'allsame}, we can adjust the order of the sequence by putting the vertices in $F$ at first and then put the vertices in $L \setminus F$ after them. The upper bound follows from the fact $F \subseteq L$ from Claim \ref{claim:FsubseteqL} and each vertex in $L \setminus F$ contributes at most $2 \Delta$ to $R$. 
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%


\begin{claim}
\label{claim:guessExpansionLbound1}
%For $\Delta=\sqrt{\eps \gamma x}$, if $x \leq \frac{\sqrt{2}-1}{2\eps} - O(1/N)$, then $|L| < \frac{1-2\Delta}{2\eps} \alpha N$.
For $\Delta=\sqrt{\gamma x \eps } + \frac{c}{N}$, if $x \in [1, \frac{\sqrt{2}-1}{2\eps} - O_\eps(1/N)]$, then $|L| < \frac{1-2\eps}{2\eps} \alpha N$.
\end{claim}
\begin{proof}
%\knote{This proof is under construction now}
Suppose after the iterations, $|L| \ge \frac{1-2\eps}{2\eps} \alpha N$.
Let $\delta=\frac{1 - 2 \Delta}{2 \eps} - x$.
%\xnote{How do we know this number is $\ge 0$? Also, how do we know that $x+\delta \geq 1$ so that we can use Lemma 2.3?}
Notice that $\delta \geq 0$. 
This is because $\Delta$ is set to be $\sqrt{\gamma x \eps} + \frac{c}{N}$ and by Lemma \ref{lem:expansion_larger}, $\gamma \leq x \eps + O_\eps(1/N)$. %\xnote{This is still not correct. If we want to use Lemma \ref{lem:expansion_larger} then we need $x \geq 1$. However the only thing we know here (at least from the conditions in the claim) is that $x \leq \frac{\sqrt{2}-1}{2\eps} - O(1/N)$. Probably need to discuss both the case of $x < 1$ and the case of $x \geq 1$. Also, even in the case of $x \geq 1$, the inequality should be $\gamma \leq x \eps + O(1/N)$.}
So $\delta=\frac{1 - 2 \Delta}{2 \eps} - x \geq \frac{1-2\eps x - \Theta_\eps(1/N)}{2\eps} - x = \frac{1}{2\eps} - 2x - \Theta_\eps(1/N)$.
Since  $\eps \leq 1/6$ and $x  \leq \frac{\sqrt{2}-1}{2\eps} - O_\eps(1/N) $, one can check that $\delta \geq 0$.
Also notice that $ x+ \delta \geq  \frac{1 }{2 \eps} - x  -\Theta_\eps(1/N) \geq 1 $ when $\eps \leq 1/6$. %\xnote{How do we know that $\gamma \leq \eps$? If $|F| > \alpha N$ it may well be possible that $\gamma > \eps$, right?}
By Claim \ref{clm:worst_expansion} and Lemma \ref{lemma:FAddtoLFirst},
we can let $L' \subseteq L$ be constituted by first adding $F$ and then $\delta \alpha N$ vertices in $L\setminus F$. 
Notice that all the unsatisfied checks are in $\Gamma(F)$, $|\Gamma(F)| \leq D|F|$, and every element in $L'\setminus F$ contributes at most $2\eps D$ vertices to $R$. 
Hence $|\Gamma(L')| \le |\Gamma(F)|+2\Delta D\cdot \delta \alpha N$. On the other hand, Lemma~\ref{lem:expansion_larger} implies $|\Gamma(L')| \ge (1-(x+\delta)\eps)D \cdot (x+\delta)\alpha N - O_\eps(1)$. Thus we have
\[
(1-(x+\delta)\eps) \cdot (x+\delta)\alpha N - O_\eps(1)\le (1-\gamma)x \alpha N + 2 \Delta \cdot \delta \alpha N.
\]
In the rest of this proof, we show that our choice of $\delta$ yields
\begin{equation}\label{eq:ineq1}
(1 - (x+\delta)\eps) \cdot (x+ \delta) - O_\eps(1/N) > (1-\gamma) x + 2 \Delta \cdot \delta.
\end{equation}
This gives a contradiction. Towards that, we rewrite  inequality~\eqref{eq:ineq1} as
\[
0 > \eps \delta^2 + (2 \eps x - 1 + 2 \sqrt{\eps \gamma x})\delta + \eps x^2 - \gamma x +  O_\eps(1/N) .
\]
When $(2 \eps x - 1 + 2 \sqrt{\eps \gamma x})^2 - 4 \eps \left( \eps x^2 -\gamma x +  O_\eps(1/N)  \right)>0$, the quadratic polynomial will be negative at $\delta_0=\frac{1 - 2 \eps x - 2 \sqrt{\eps \gamma x}}{2\eps}=\delta $. To verify $(2 \eps x - 1 + 2 \sqrt{\eps \gamma x})^2 - 4 \eps \left( \eps x^2 -\gamma x +  O_\eps(1/N)  \right)>0$, we set $c=\eps x$ and rewrite it as
\[
(2c - 1 + 2 \sqrt{\gamma c})^2 - 4 c^2 + 4 \gamma c -  O_\eps(1/N) >0.
\]
This is equivalent to
\[
8 \gamma c + (8c -4 ) \sqrt{\gamma c} + 1 - 4c  - O_\eps(1/N) > 0 \Rightarrow 8(\sqrt{\gamma c} +\frac{2c-1}{4})^2  - O_\eps(1/N) + 1 - 4c - 8(\frac{2c-1}{4})^2 > 0.
\]
%\textcolor{red}{Xue: We may wanna handle the extra $O(1/N)$ term here. At least, we need to change $\leq$ to $<$.}
%\knote{I think the $O(1/N)$ term can be obsorbed by the $8(\sqrt{\gamma c} +\frac{2c-1}{4})^2$? }
%\knote{I concede that with a $-O(1/N)$ term in $x$ the analysis will be much easier}
When $c=\eps x \leq \frac{\sqrt{2}-1}{2} - O_\eps(1/N)$, i.e. $x \leq \frac{\sqrt{2}-1}{2\eps} - O_\eps(1/N)$,
%\xnote{Doesn't the analysis imply that the $O()$ in $x$ depends on $\eps$? Then we cannot simply write it as $O()$ because $\eps$ appears explicity in the first term.} 
the residue $1 - 4c - 8(\frac{2c-1}{4})^2 -O_\eps(1/N)>0$. 
So the inequality holds.
\end{proof}

\begin{claim}
\label{claim:guessExpansionLbound2}
For $\Delta=\eps$, if  $x \leq \frac{1-2\eps}{4\eps} - O_\eps(1/N)$, then $|L| < \frac{1-2\eps}{2\eps} \alpha N$.
\end{claim}
%\textcolor{red}{This proof assumes $x+\delta \ge 1$. But one can bound the case $x+\delta \le 1$ by a similar argument.}
\begin{proof}

Suppose $|L| \geq \frac{1-2\eps}{2\eps} \alpha N$.
Consider $L'\subseteq L$ with $|L'| =  \frac{1-2\eps}{2\eps} \alpha N$.
Let $\delta = \frac{1-2\eps}{2\eps} - x$. 
%Notice that $\delta >0$ since we only need to consider every $x\leq \frac{1-2\eps}{4\eps} - O(1)$.
%\xnote{Again, need to verify that $\delta \geq 0$ and $x+\delta \geq 1$.}
Notice that $\delta \geq 0$ because    $x \leq  \frac{1-2\eps}{4\eps} - O_\eps(1/N)$.
Also $x+ \delta \geq 1$ since $\eps \leq 1/8$.
By Lemma \ref{lem:expansion_larger}, $|\Gamma(L')| \geq (1-(x+\delta)\eps)D |L'| - O_\eps(1)$.
By Lemma \ref{lemma:FAddtoLFirst} we can consider $L'$ as being constituted by first adding all elements in $F$ and then add another $\delta \alpha N$ elements by the algorithm.
Notice that all the unsatisfied checks are in $\Gamma(F)$, $|\Gamma(F)| \leq D|F|$, and every element in $L'\setminus F$ contributes at most $2\eps D$ vertices to $R$. 
Hence $|\Gamma(L')| \leq D|F| + 2\eps D \delta \alpha N$.
So we have
\[
(1-(x+\delta)\eps)D |L'| - O_\eps(1) \leq  |\Gamma(L')| \leq D|F| + 2\eps D \delta \alpha N
\]
Thus
\[
(1-(x+\delta)\eps) \cdot (x+\delta) - O_\eps(1/N) \le x + 2 \eps \delta.
\]
%\xnote{Need to explain the above inequality in more details.}
So this is equivalent to
\[
(1- 2\eps - \eps (x+\delta))(x+\delta)  - O_\eps(1/N)  \le (1-2\eps) x
\]
Recall that $\delta+x=\frac{1 -2 \eps}{2\eps}$. 
%\xnote{This sentence is useless, we already fixed $\delta$.} 
To get a contradiction, we only need 
\[
(1-2\eps) x < (1-2\eps)^2/4\eps - O(1/N).
\]
Namely $x \leq \frac{1-2\eps}{4\eps} - O_\eps(1/N)$.


%If $x + \delta < 1$, then because $\eps \leq 1/6 < 1/4$, we have $\frac{1-2\eps}{2\eps} \geq 1 > x+ \delta = |L|$.

\end{proof}

\begin{proofof}{Theorem \ref{thm:guessexpansion}}
One of our enumerations correctly predicts  $|F|$ and  $|\Gamma(F)|$.
Consider   Algorithm \ref{alg:decoding_small_eps} under this enumeration.
After the function $\mathrm{Find}$, all the errors are in $L$ by Claim \ref{claim:FsubseteqL}. 
Now we bound $|L|$. 
When $x  <  1$, then $\Delta = \eps$ in the algorithm.
By Claim \ref{claim:guessExpansionLbound2},  $|L| \leq  \frac{1-2\eps}{2\eps}\alpha N $, as long as $x \leq \frac{1-2\eps}{4\eps} - O_\eps(1/N)$.
%But when $N$ is large enough this number is at least $\frac{1-2\eps}{4\eps} - 1$. 
When $x \geq 1$, to bound $|L|$, we now just need to pick the smaller bound of $x$ from Claim   \ref{claim:guessExpansionLbound1} and Claim   \ref{claim:guessExpansionLbound2}.
If $\eps < \frac{3-2\sqrt{2}}{2} $, then $\frac{\sqrt{2}-1}{2\eps} < \frac{1-2\eps}{4\eps}$. 
So by Claim   \ref{claim:guessExpansionLbound1} and Claim   \ref{claim:guessExpansionLbound2}  when $x \in [1,  \frac{\sqrt{2}-1}{2\eps} - O_\eps(1/N)]$ we have $|L| < \frac{1-2\eps}{2\eps}\alpha N  $.
If $\eps \in [\frac{3-2\sqrt{2}}{2}, 1/8]$, then $\frac{\sqrt{2}-1}{2\eps} \geq \frac{1-2\eps}{4\eps}$.
By Claim   \ref{claim:guessExpansionLbound1} and Claim   \ref{claim:guessExpansionLbound2} , when 
$x \in [1,  \frac{1-2\eps}{4\eps} - O_\eps(1/N)]$, we have $|L| < \frac{1-2\eps}{2\eps} \alpha N$. 
%\xnote{With the modification in the algorithm and in Claim   \ref{claim:guessExpansionLbound1}, this part now needs more explanation. Specifically, Claim \ref{claim:guessExpansionLbound1} now only works for $x \ge 1$, so we cannot simply combine both claims to get a bound like $x \leq  \frac{\sqrt{2}-1}{2\eps} - O(1/N)$ or $x \leq   \frac{1-2\eps}{4\eps} - O(1/N)$. Need to explain that when $x < 1$, we always use $\Delta=\eps$ and thus this case is covered by Claim   \ref{claim:guessExpansionLbound2}.}
%\knote{This is indeed an issue. But if we modify like this, there is still  an issue, i.e. in claim \ref{claim:guessExpansionLbound2}, the bound of $x$ is less than $1$. But we need it to be exactly $1$. We can let $\eps < 1/6-O(1/N)$ to avoid this issue, but then there is a gap between this and $1/6$.}
Since the expander is an $(\alpha N, (1-\eps)D)$ expander,  by Theorem \ref{thm:decfromerasures}, one can correct all the errors efficiently using $L$ (as the erasure area) and the corrupted codeword.
  
\end{proofof}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> backup4.tex <==
\section{Improved Unique Decoding  for  $\eps \leq 1/8$}\label{sec:improve_decoding}

 


Consider the expander code on an $(\alpha N, (1-\eps)D)$ bipartite expander $G$. 
For the case of $\eps \le 1/8$ we provide an efficient algorithm,  i.e. Algorithm~\ref{alg:decoding_small_eps}, to decode more errors.
It is again by guessing the expansion of the corrupted entries. 


\begin{algorithm}[H]
\caption{Decoding Algorithm for $\eps\le 1/8$}\label{alg:decoding_small_eps}
\begin{algorithmic}[1]
\Function{Decoding}{$y \in \mathbf{F}_2^N$ }
\State Enumerate $\tilde{x}$ from $\{ \eta , 2\eta , \ldots, \lceil\frac{1}{4\eps \eta } \rceil \eta  \}$ and enumerate $\tilde{\gamma}\tilde{x}$ from $\{ \eta , 2\eta , \ldots, \lceil\frac{1}{\eta } \rceil \eta  \}$, where $\eta<1$ is a small enough constant.
	    \If{$\tilde{\gamma} \tilde{x}\ge \eps + 3\eta$ and $\tilde{x} \geq 1-\eta$}
	        \State $\Delta \gets \sqrt{\tilde{\gamma} \tilde{x} \eps}$.
	    \Else
	        \State $\Delta  \gets \eps$
	    \EndIf
	    \State $L \gets $ \Call{Find}{$y \in \mathbf{F}_2^n$ and $\Delta$}
	    \State Apply Theorem \ref{thm:decfromerasures} with $L$ and $y$ to get a codeword $C'$.
	    \State \Return $C'$ if distance between $C'$ and $y$ is $\le \frac{1-2\eps}{4 \eps}\alpha N $ where the distance comes from Theorem~\ref{thm:dist_expander}.
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:guessexpansion}
Consider the expander code defined by an $(\alpha N, (1-\eps)D)$ expander.
For $\eps< \frac{3-2\sqrt{2}}{2}$, there is a linear time decoding algorithm with  radius $\frac{\sqrt{2}-1}{2\epsilon} \alpha N -O_{\eps}(1) $. 
Next for $\eps \in [\frac{3-2\sqrt{2}}{2}, 1/8]$, 
there is a linear time decoding algorithm with   radius $\frac{1-2\eps}{4\eps} \alpha N - O_{\eps}(1)$.

\end{theorem}



We prove the correctness of Algorithm~\ref{alg:decoding_small_eps} in the rest of this section. Again $F$ always denotes the subset of entries that are flipped by the adversary. 
Again let $F$ be the set of corruptions and assume $|F| = x\alpha N$, $|\Gamma(F)| = (1-\gamma)D|F|$.
Since we enumerate $\tilde{x}$   and $\tilde{\gamma}$, one pair of them is such that $x \in [\tilde{x} , \tilde{x}+ \eta], \gamma x \in [\tilde{\gamma}\tilde{x} ,\tilde{\gamma}\tilde{x}+ \eta]$.
Now we only consider this pair $\tilde{x}$ and $\tilde{\gamma}$  in the following analysis.

First of all, we bound the expansion of all subsets in $F$.
\begin{claim}\label{clm:worst_expansion}
Our choice of $\Delta$ always satisfies that
\[
\forall F' \subseteq F, F'\neq \emptyset, |\Gamma(F')| \ge (1-\Delta) \cdot D |F'|.
\]
\end{claim}
\begin{proof}
Let $F'$ be the subset of $F$ with the worst expansion and denote $|F'| = x' \cdot \alpha N$. 

If $\tilde{x} < 1-\eta$, then $x' < 1 $.
So then $|\Gamma(F')| \ge (1- \eps) \cdot D |F'|$ by the expansion property. 
This is at least $(1-\Delta)D|F'|$ since $\Delta =    \eps$ in the algorithm.

If $\tilde{x} \geq 1-\eta$, then $x' \geq 1-\eta$.
We have two cases.
First case, $x' \in [1-\eta, 1]$. Then $|\Gamma(F')| \ge (1 - \eps )\cdot D |F'|$ by the expansion property.
If $\tilde{\gamma} \tilde{x}\ge \eps + 3\eta $, then notice that this is at least $(1-\Delta)D|F'|$ since $\Delta = \sqrt{\tilde{x}\tilde{\gamma}\eps}\geq \sqrt{(\eps+3\eta)\eps} \geq  \eps $.
Else, we run into the second branch and $\Delta = \eps$.


Second case,   $x'\geq 1$. 
We consider the collisions   in $\Gamma(F)$ and $\Gamma(F')$.
~By collision we mean that given an arbitrary order of the edges, if one edge in this order has its right ending the same as any other edge in previous of it, then this is called a collision. 
Since $F'$ is  of size $x' \cdot \alpha N$, by Lemma \ref{lem:expansion_larger}, $|\Gamma(F')| \ge (1-x' \cdot \eps) D \cdot x' \alpha N - O_\eps(1)$. So we have that the total number of collisions for edges with left endings in $F'$ is at most the total number of collisions for edges with left endings in $F$, because a collision  in $\Gamma(F')$ is also a collision in $\Gamma(F)$, according to an arbitrary order of all edges connected to vertices in $F$. 
So
\[
x' \alpha N \cdot (x' \cdot \eps)D  + O_\eps(1) \le |F| \cdot \gamma D.
\]
This implies $x' \cdot \eps \le \sqrt{\gamma x\eps } $.
When $\tilde{\gamma} \tilde{x}\ge \eps + 3\eta $, $  \sqrt{\gamma x\eps }  \leq \Delta - \Theta(\eta)$
because $\gamma x \leq \tilde{\gamma}\tilde{x} + \eta$, $\eps \leq \tilde{\gamma}\tilde{x}  - 3\eta $.
Hence $|\Gamma(F')| \ge (1-\Delta+ \Theta(\eta)) D \cdot |F'| - O_\eps(1) \geq  (1-\Delta) D \cdot |F'|$, noticing $|F'|= x'\alpha N \geq \alpha N$.
When $\tilde{\gamma} \tilde{x} < \eps + 3\eta $, $  \sqrt{\gamma x\eps }   \leq \eps -\Theta(\eta).$
Hence again $|\Gamma(F')| \ge (1-\eps+ \Theta(\eta)) D \cdot |F'| - O_\eps(1) \geq  (1-\eps) D \cdot |F'|$, noticing $|F'|= x'\alpha N \geq \alpha N$.
\end{proof}

Given the guarantee in Claim~\ref{clm:worst_expansion}, one can show that $L$ contains all the errors.
%\textcolor{blue}{Xue: Clarify what we mean ``correct"?}
\begin{claim}
\label{claim:FsubseteqL}
After step 9 in Algorithm~\ref{alg:decoding_small_eps}, we have $F\subseteq L$.
\end{claim}

\begin{proof}
By Claim \ref{clm:worst_expansion}, $\forall F' \subseteq F, |\Gamma(F')| \ge (1-\Delta) \cdot D |F'|$.
So $\forall F' \subseteq F, |\Gamma^1(F')| \ge (1-2\Delta) \cdot D |F'|$.
By Lemma \ref{lemma:all_errors_in_L}, we know $F\subseteq L$ after \textsc{Find}.
\end{proof}

%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}
Suppose there are $F\setminus L = B \neq \emptyset$. 
Since $B\subseteq F$, by Claim \ref{clm:worst_expansion}, $|\Gamma(B)| \geq (1-\Delta)D|B|$.
So the number of unique neighbors is at least $(1-2\Delta)D|B|$.
Hence there is a $v\in B$ which has at least $(1-2\Delta)D$ unique neighbors.
But $v$ is not in $L$, meaning it has $<(1-2\Delta)D$ neighbors in $R$.
So it has a unique neighbor which is not in $R$.
This is a contradiction since this unique neighbor corresponds to an unsatisfied check which has to be in $R_0 \subseteq R$. 
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%
Then we calculate the decoding radius and the size of $L$. 


%%%%%%%%%%%%%%%%%%% The following claim seems a bit unflexible to use because when we need it usually we already argued that L is generated by first adding $F$ then other vertices. Also it can only work for those moments where |L| \geq |F| 
\iffalse
\begin{claim}\label{clm:upper_bound_neighbors}
For both $\Delta=\eps$ and $\Delta=\sqrt{\eps \gamma x}$, $|\Gamma(L)| \le |\Gamma(F)| + 2 \Delta D \cdot |L \setminus F|$.
\end{claim}
\begin{proof}
Let $(v_1,\ldots,v_{|L|})$ be the sequence of vertices added to $L$ in the while. By Lemma \ref{lemma:L'allsame}, we can adjust the order of the sequence by putting the vertices in $F$ at first and then put the vertices in $L \setminus F$ after them. The upper bound follows from the fact $F \subseteq L$ from Claim \ref{claim:FsubseteqL} and each vertex in $L \setminus F$ contributes at most $2 \Delta$ to $R$. 
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%


\begin{claim}
\label{claim:guessExpansionLbound1}
 
For $\Delta=\sqrt{\tilde{\gamma}\tilde{x} \eps }  $, if $x \in [1, \frac{\sqrt{2}-1}{2\eps} - O_\eps(1/N)]$, then $|L| < \frac{1-2\eps}{2\eps} \alpha N$.
\end{claim}
\begin{proof}
Suppose after the iterations, $|L| \ge \frac{1-2\eps}{2\eps} \alpha N$.
Let $\delta=\frac{1 - 2 \sqrt{\gamma x \eps}}{2 \eps} - x$.
Notice that $\delta \geq 0$. 
This is because   by Lemma \ref{lem:expansion_larger} , $\gamma \leq x \eps + O_\eps(1/N)$ when $x\geq 1$. 
So $\delta=\frac{1 - 2 \Delta}{2 \eps} - x \geq \frac{1-2\eps x -O_\eps(1/N)}{2\eps} - x = \frac{1}{2\eps} - 2x -O_\eps(1/N)$.
Since  $\eps \leq 1/8$, $x  \leq \frac{\sqrt{2}-1}{2\eps} - O_\eps(1/N) $, one can check that $\delta \geq 0$.
Also notice that $ x+ \delta \geq  \frac{1 }{2 \eps} - x  -O_\eps(1/N)\geq 1 $ when $\eps \leq 1/8$. 
By Claim \ref{clm:worst_expansion} and Lemma \ref{lemma:FAddtoLFirst},
we can let $L' \subseteq L$ be constituted by first adding $F$ and then $\delta \alpha N$ vertices in $L\setminus F$. 
Notice that all the unsatisfied checks are in $\Gamma(F)$, $|\Gamma(F)| \leq D|F|$, and every element in $L'\setminus F$ contributes at most $2\eps D$ vertices to $R$. 
Hence $|\Gamma(L')| \le |\Gamma(F)|+2\Delta D\cdot \delta \alpha N$. On the other hand, Lemma~\ref{lem:expansion_larger} implies $|\Gamma(L')| \ge (1-(x+\delta)\eps)D \cdot (x+\delta)\alpha N - O_\eps(1)$. Thus we have
\[
(1-(x+\delta)\eps) \cdot (x+\delta)\alpha N - O_\eps(1)\le (1-\gamma)x \alpha N + 2 \Delta \cdot \delta \alpha N.
\]
Notice that $\Delta \leq \sqrt{\gamma x \eps}$, so the R.H.S. is at most  $(1-\gamma)x \alpha N + 2 \sqrt{\gamma x \eps} \cdot \delta \alpha N$.
In the rest of this proof, we show that our choice of $\delta$ yields
\begin{equation}\label{eq:ineq1}
(1 - (x+\delta)\eps) \cdot (x+ \delta) - O_\eps(1/N) > (1-\gamma) x + 2 \sqrt{\gamma x \eps}\cdot \delta.
\end{equation}
This gives a contradiction. Towards that, we rewrite  inequality~\eqref{eq:ineq1} as
\[
0 > \eps \delta^2 + (2 \eps x - 1 + 2\sqrt{\gamma x \eps})\delta + \eps x^2 - \gamma x +  O_\eps(1/N) .
\]
When $(2 \eps x - 1 + 2 \sqrt{\gamma x \eps})^2 - 4 \eps \left( \eps x^2 -\gamma x +  O_\eps(1/N)  \right)>0$, the quadratic polynomial will be negative at $\delta_0=\frac{1 - 2 \eps x - 2 \sqrt{\gamma x \eps}}{2\eps}=\delta $. 
To verify $(2 \eps x - 1 + 2 \sqrt{\gamma x \eps})^2 - 4 \eps \left( \eps x^2 -\gamma x +  O_\eps(1/N)  \right)>0$, we set $c=\eps x$ and rewrite it as
\[
(2c - 1 + 2 \sqrt{\gamma c})^2 - 4 c^2 + 4 \gamma c -  O_\eps(1/N) >0.
\]
This is equivalent to
\[
8 \gamma c + (8c -4 ) \sqrt{\gamma c} + 1 - 4c  - O_\eps(1/N) > 0 \Rightarrow 8(\sqrt{\gamma c} +\frac{2c-1}{4})^2  - O_\eps(1/N) + 1 - 4c - 8(\frac{2c-1}{4})^2 > 0.
\]
%\textcolor{red}{Xue: We may wanna handle the extra $O(1/N)$ term here. At least, we need to change $\leq$ to $<$.}
%\knote{I think the $O(1/N)$ term can be obsorbed by the $8(\sqrt{\gamma c} +\frac{2c-1}{4})^2$? }
%\knote{I concede that with a $-O(1/N)$ term in $x$ the analysis will be much easier}
When $c=\eps x \leq \frac{\sqrt{2}-1}{2} - O_\eps(1/N)$, i.e. $x \leq \frac{\sqrt{2}-1}{2\eps} - O_\eps(1/N)$,
%\xnote{Doesn't the analysis imply that the $O()$ in $x$ depends on $\eps$? Then we cannot simply write it as $O()$ because $\eps$ appears explicity in the first term.} 
the residue $1 - 4c - 8(\frac{2c-1}{4})^2 -O_\eps(1/N)>0$. 
So the inequality holds.
\end{proof}

\begin{claim}
\label{claim:guessExpansionLbound2}
For $\Delta=\eps$, if  $x \leq \frac{1-2\eps}{4\eps} - O_\eps(1/N)$, then $|L| < \frac{1-2\eps}{2\eps} \alpha N$.
\end{claim}
%\textcolor{red}{This proof assumes $x+\delta \ge 1$. But one can bound the case $x+\delta \le 1$ by a similar argument.}
\begin{proof}

Suppose $|L| \geq \frac{1-2\eps}{2\eps} \alpha N$.
Consider $L'\subseteq L$ with $|L'| =  \frac{1-2\eps}{2\eps} \alpha N$.
Let $\delta = \frac{1-2\eps}{2\eps} - x$. 
%Notice that $\delta >0$ since we only need to consider every $x\leq \frac{1-2\eps}{4\eps} - O(1)$.
%\xnote{Again, need to verify that $\delta \geq 0$ and $x+\delta \geq 1$.}
Notice that $\delta \geq 0$ because    $x \leq  \frac{1-2\eps}{4\eps} - O_\eps(1/N)$.
Also $x+ \delta \geq 1$ since $\eps \leq 1/8$.
By Lemma \ref{lem:expansion_larger}, $|\Gamma(L')| \geq (1-(x+\delta)\eps)D |L'| - O_\eps(1)$.
By Lemma \ref{lemma:FAddtoLFirst} we can consider $L'$ as being constituted by first adding all elements in $F$ and then add another $\delta \alpha N$ elements by the algorithm.
Notice that all the unsatisfied checks are in $\Gamma(F)$, $|\Gamma(F)| \leq D|F|$, and every element in $L'\setminus F$ contributes at most $2\eps D$ vertices to $R$. 
Hence $|\Gamma(L')| \leq D|F| + 2\eps D \delta \alpha N$.
So we have
\[
(1-(x+\delta)\eps)D |L'| - O_\eps(1) \leq  |\Gamma(L')| \leq D|F| + 2\eps D \delta \alpha N
\]
Thus
\[
(1-(x+\delta)\eps) \cdot (x+\delta) - O_\eps(1/N) \le x + 2 \eps \delta.
\]
%\xnote{Need to explain the above inequality in more details.}
So this is equivalent to
\[
(1- 2\eps - \eps (x+\delta))(x+\delta)  - O_\eps(1/N)  \le (1-2\eps) x
\]
Recall that $\delta+x=\frac{1 -2 \eps}{2\eps}$. 
%\xnote{This sentence is useless, we already fixed $\delta$.} 
To get a contradiction, we only need 
\[
(1-2\eps) x < (1-2\eps)^2/4\eps - O(1/N).
\]
Namely $x \leq \frac{1-2\eps}{4\eps} - O_\eps(1/N)$.


%If $x + \delta < 1$, then because $\eps \leq 1/6 < 1/4$, we have $\frac{1-2\eps}{2\eps} \geq 1 > x+ \delta = |L|$.

\end{proof}

\begin{proofof}{Theorem \ref{thm:guessexpansion}}
One of our enumerations has $\tilde{x}$ and $\tilde{\gamma}\tilde{x}$ such that $x \in [\tilde{x} , \tilde{x}+ \eta], \gamma x \in [\tilde{\gamma}\tilde{x} ,\tilde{\gamma}\tilde{x}+ \eta]$.
Consider   Algorithm \ref{alg:decoding_small_eps} under this enumeration.
After the function $\mathrm{Find}$, all the errors are in $L$ by Claim \ref{claim:FsubseteqL}. 
Now we bound $|L|$. 
When $\tilde{x}  <  1 - \eta$ we know $x<1 $ and $\Delta = \eps$ in the algorithm.
By Claim \ref{claim:guessExpansionLbound2},  $|L| \leq  \frac{1-2\eps}{2\eps}\alpha N $, as long as $x \leq \frac{1-2\eps}{4\eps} - O_\eps(1/N)$.
%But when $N$ is large enough this number is at least $\frac{1-2\eps}{4\eps} - 1$. 
When $\tilde{x} \geq 1$, we know $x\geq 1$. 
To bound $|L|$, we now just need to pick the smaller bound of $x$ from Claim   \ref{claim:guessExpansionLbound1} and Claim   \ref{claim:guessExpansionLbound2}.
If $\eps < \frac{3-2\sqrt{2}}{2} $, then $\frac{\sqrt{2}-1}{2\eps} < \frac{1-2\eps}{4\eps}$. 
So by Claim   \ref{claim:guessExpansionLbound1} and Claim   \ref{claim:guessExpansionLbound2}  when $x \in [1,  \frac{\sqrt{2}-1}{2\eps} - O_\eps(1/N)]$ we have $|L| < \frac{1-2\eps}{2\eps}\alpha N  $.
If $\eps \in [\frac{3-2\sqrt{2}}{2}, 1/8]$, then $\frac{\sqrt{2}-1}{2\eps} \geq \frac{1-2\eps}{4\eps}$.
So by Claim   \ref{claim:guessExpansionLbound1} and Claim   \ref{claim:guessExpansionLbound2} , when 
$x \in [1,  \frac{1-2\eps}{4\eps} - O_\eps(1/N)]$, we have $|L| < \frac{1-2\eps}{2\eps} \alpha N$. 
%\xnote{With the modification in the algorithm and in Claim   \ref{claim:guessExpansionLbound1}, this part now needs more explanation. Specifically, Claim \ref{claim:guessExpansionLbound1} now only works for $x \ge 1$, so we cannot simply combine both claims to get a bound like $x \leq  \frac{\sqrt{2}-1}{2\eps} - O(1/N)$ or $x \leq   \frac{1-2\eps}{4\eps} - O(1/N)$. Need to explain that when $x < 1$, we always use $\Delta=\eps$ and thus this case is covered by Claim   \ref{claim:guessExpansionLbound2}.}
%\knote{This is indeed an issue. But if we modify like this, there is still  an issue, i.e. in claim \ref{claim:guessExpansionLbound2}, the bound of $x$ is less than $1$. But we need it to be exactly $1$. We can let $\eps < 1/6-O(1/N)$ to avoid this issue, but then there is a gap between this and $1/6$.}
Since the expander is an $(\alpha N, (1-\eps)D)$ expander,  by Theorem \ref{thm:decfromerasures}, one can correct all the errors efficiently using $L$ (as the erasure area) and the corrupted codeword.
  
\end{proofof}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

